Correctness and Performance for Stateful Chained Network Functions

Network functions virtualization (NFV) allows operators to employ NF chains to realize custom policies, and dynamically add instances to meet demand or for failover. NFs maintain detailed per- and cross-flow state which needs careful management, especially during dynamic actions. Crucially, state management must: (1) ensure NF chain-wide correctness and (2) have good performance. To this end, we built \name, an NFV framework that leverages an external state store coupled with state management algorithms and metadata maintenance for correct operation even under a range of failures. Our evaluation shows that CHC can support ~10Gbps per-NF throughput and <0.6mus increase in median per-NF packet processing latency, and chain-wide correctness at little additional cost.

==> challenges.tex <==
\section{Challenges}
Following are the key challenges in designing a framework for managing distributed NFs in order to ensure elastic scaling and high availability.  In the rest of this section, we  discuss the challenges in the context of distributed NFs.

\subsection{Elastic scaling}
To support elastic scaling, a distributed NF management framework must be able to spin up new instances of NF and distribute input network traffic among all the instances. Just spinning up new instances and re-distributing the load among them is not enough, scaling NFs bring additional challenges to the management of internal state; unlike other distributed applications where there is a clear notion of transactions, most of the time the notion of transactions does not apply to NFs. In addition to that NFs are stateful, they may create or may update the state on every packet. Some of these states apply to traffic originating from different users, networks or traffic classes.  To ensure output equivalence while redistributing the input network traffic among different instances, handling of internal state is required. To scale a NF efficiently, the framework is required to provide the following:

\begin{enumerate}
\item {\bf Scope-aware input partitioning:} A framework must be able to partition the network traffic among the NFs in such a way that the processing of traffic in each partition has minimal dependence on the processing of the traffic in another partition. For example, if an IDS maintains a state associated with the host, then the framework should try to process all the traffic of a particular host on a single instance.

\item {\bf State Transfer:}
When the input traffic is moved from one NF to another, the internal state is also required to move. This state is built at run-time and is required for the processing of the network traffic e.g. A NAT maintains an IP/port mapping between private and public network. The absence of this state at the new NF could result in the termination of a network connection.

\item {\bf State sharing:}
In addition to transferring the internal state, NFs need to share states among different instances. NFs maintain states which are shared among different network flows, e.g. Bro - an IDS maintains states per host. For every host, it keeps track of the number of active connections. When the input traffic is processed by multiple instances, the shared internal state needs to be available to all of those instances.
\end{enumerate}

\subsection{Fault tolerance}
Failures are inevitable in distributed systems, so the framework must recover fast from the failure. The continuous operator model of NFs along with internal state makes it difficult to handle failure. The framework has to (1) recover the unprocessed input, which was buffered at the failed instance. (2) recover the internal state. (3) resume the processing of input from where it failed. The instance would have failed after updating some of the shared state, updating the same state again could cause an inconsistent state. 

\subsection{Straggler mitigation}
In a distributed framework, instances could be slow because of hardware or software bugs. Handling straggler is not an easy task, unlike typical stream processing applications, a VNF framework cannot perform a speculative execution because instances not only maintain states but they also share those states. A naive speculative execution could end up performing duplicate operations, e.g. updating the packet count more than once for a single input.

\subsection{Avoid packet re-parsing}
Service chain is used to meet the high level performance and security objectives. In some cases, multiple NFs in the service chain extract the same information from the packet header, e.g. re-parsing the same protocol header or reconstructing the same session. NFs must reuse the information parsed or constructed by one instance to avoid resource wastage.

\subsection{Ensure packet ordering}
\label{trojanexample}
Some NFs require ordering across different flows for their processing. For example, the multistep trojan detector described in ~\cite{lorenzos_work} uses across flow state analysis to identify a trojan. The IDS leverages the fact that the particular trojan perform following sequence of steps: (1) opens an SSH connection; (2) downloads an HTML file and a ZIP and EXE file over an FTP connection; (3) generate IRC activity. The order of the steps is relevant, any different order does not indicate the fingerprint of the trojan. Ensuring ordering across flows, when the flows are processed by different instances is hard because synchronizing clock is expensive. A naive approach to ensure ordering across flows would be to use scope-aware partitioning to process all the flows which have ordering requirement on a single instance. However, this limits the ability of the framework to scale. A framework must ensure ordering across the flow, if required.

\subsection{Dynamic service chaining}
Network operators use NFs in service chains to meet high-level policy objectives, such as performance, resource monitoring and security objective. For example, a policy could be that all incoming traffic passes through a Firewall, followed by a caching proxy, and a load balancer. Additionally, a network operator may also want to dynamically add and or remove an NFs from the service chain in response to changes in the network traffic. For example, a deep packet inspection (DPI) engine may need to be added to the chain for further inspection if the firewall detects some malicious activity. Similarly, an NF may be needed to be removed from the chain when it is no longer needed to reduce packet latency and resource wastage.

\subsection{Efficient placement}
The framework must not only reduce cross rack traffic, but also avoid unnecessary usage of switch capacity by efficiently placing the instances in the rack. In addition to this, the instance may have hardware requirements for their operation such as remote memory access (RDMA), encryption engine or hardware accelerator. Prior work \cite{gember2013stratos,E2} has looked at efficient placement, in this paper, we do not focus on efficient placement.



==> otherrelatedwork.tex <==
\section{StatelessNF and Some other Works}

\aditya{talk about statelessNF in detail here. and then about other papers.} \junaid{updated}
\JK{  
We note that StatelessNF~\cite{statelessnf} which first 
advocates for externalizing state claims to support R1 as well. However,unfortunately it does not ensure atomic state update nor does it have
have a state rollback mechanism. This can lead to an inconsistent state when an NF fails after updating some of the state
objects. Moreover, it does not provide support for updating shared states. To support consistent updates to shared states, it
requires locks, which can significantly degrades the performance. Unlike \name, low latency networks (RDMA or Infiniband) are crucial for the performance of StatelessNF.



==> package.tex <==
%\usepackage{oneinchmargins,doublespace,times}
\usepackage{oneinchmargins}
\usepackage{times}
\usepackage{graphicx}
\usepackage{url}
%\usepackage{color}
\usepackage{float}
\usepackage{verbatim}
\usepackage{authblk}
\usepackage{calc}
\usepackage{soul}

%\usepackage[]{hyperref}
%\usepackage[bookmarks=false,breaklinks]{hyperref}
%\usepackage[hyphenbreaks]{breakurl}


\usepackage{setspace}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{wrapfig}
\usepackage{alltt}
\usepackage{epstopdf}
%\usepackage{subfigure}
%\usepackage{pifont}

% for tables
\usepackage{booktabs}
\usepackage{threeparttable}


%\usepackage{bbding}
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
%\usepackage{mathtools}
%\usepackage{listings}
\usepackage{algorithm}
\usepackage{algorithmic}
%\usepackage[noend]{algpseudocode}

\usepackage{tabularx}

\usepackage{fancyvrb}
\usepackage[normalem]{ulem} % for strike out,  \em and \sout are now strikes, use \it for italic
\renewcommand{\ttdefault}{cmtt}

%\usepackage{colortbl} % for table color
\usepackage{pstricks} % for gray hline
%\input{colortab} % for gray hline (must include pstricks)
\usepackage{array}

\usepackage{textcomp}

\usepackage{enumerate}
\usepackage[shortlabels]{enumitem}
\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

\usepackage[normalem]{ulem}  % for strike through



==> paper - Copy/abstract.tex <==

%\begin{abstract}


\noindent
{\bf Abstract:} Network functions virtualization (NFV) allows
operators to employ NF chains to realize custom policies, and
dynamically add instances to meet demand or for failover. NFs maintain
detailed per- and cross-flow state which needs careful management,
especially during dynamic actions. Crucially, state management must:
(1) ensure NF {\em chain-wide} correctness and (2) have good
performance. To this end, we built
\name, an NFV framework that leverages an external state store
coupled with state management algorithms and metadata maintenance for
correct operation even under a range of failures. Our evaluation shows
that \name can support $\sim$10Gbps per-NF throughput and $<0.6\mu$s increase in \CR{median} per-NF packet processing latency, and chain-wide correctness at little additional cost.

%\end{abstract}
%% While there
%% are many existing NFV frameworks today


%%  \aditya{NEED TO UPDATE Network Functions Virtualization (NFV)
%%    promises network operators a great flexibility in managing their
%%    networks by enabling on-demand scaling and providing high
%%    availability in case of failure.  However, these features come at a
%%    price - network function (NF) developers need to provide inbuilt
%%    support for scalability and high availability. Providing this
%%    support is tedious, and is slowing down the wider adoption of
%%    NFV. Simplifying this process is key for wider proliferation of
%%    NFV. To this end, we design a generic, and network function
%%    independent framework that makes it easier for developers to build
%%    scalable and highly available NFs. We offload the complexity of
%%    providing these features to the framework at a minimal overhead,
%%    similar to frameworks for cloud computing applications.}
 



==> paper - Copy/challenges.tex <==
\section{Challenges}
Following are the key challenges in designing a framework for managing distributed NFs in order to ensure elastic scaling and high availability.  In the rest of this section, we  discuss the challenges in the context of distributed NFs.

\subsection{Elastic scaling}
To support elastic scaling, a distributed NF management framework must be able to spin up new instances of NF and distribute input network traffic among all the instances. Just spinning up new instances and re-distributing the load among them is not enough, scaling NFs bring additional challenges to the management of internal state; unlike other distributed applications where there is a clear notion of transactions, most of the time the notion of transactions does not apply to NFs. In addition to that NFs are stateful, they may create or may update the state on every packet. Some of these states apply to traffic originating from different users, networks or traffic classes.  To ensure output equivalence while redistributing the input network traffic among different instances, handling of internal state is required. To scale a NF efficiently, the framework is required to provide the following:

\begin{enumerate}
\item {\bf Scope-aware input partitioning:} A framework must be able to partition the network traffic among the NFs in such a way that the processing of traffic in each partition has minimal dependence on the processing of the traffic in another partition. For example, if an IDS maintains a state associated with the host, then the framework should try to process all the traffic of a particular host on a single instance.

\item {\bf State Transfer:}
When the input traffic is moved from one NF to another, the internal state is also required to move. This state is built at run-time and is required for the processing of the network traffic e.g. A NAT maintains an IP/port mapping between private and public network. The absence of this state at the new NF could result in the termination of a network connection.

\item {\bf State sharing:}
In addition to transferring the internal state, NFs need to share states among different instances. NFs maintain states which are shared among different network flows, e.g. Bro - an IDS maintains states per host. For every host, it keeps track of the number of active connections. When the input traffic is processed by multiple instances, the shared internal state needs to be available to all of those instances.
\end{enumerate}

\subsection{Fault tolerance}
Failures are inevitable in distributed systems, so the framework must recover fast from the failure. The continuous operator model of NFs along with internal state makes it difficult to handle failure. The framework has to (1) recover the unprocessed input, which was buffered at the failed instance. (2) recover the internal state. (3) resume the processing of input from where it failed. The instance would have failed after updating some of the shared state, updating the same state again could cause an inconsistent state. 

\subsection{Straggler mitigation}
In a distributed framework, instances could be slow because of hardware or software bugs. Handling straggler is not an easy task, unlike typical stream processing applications, a VNF framework cannot perform a speculative execution because instances not only maintain states but they also share those states. A naive speculative execution could end up performing duplicate operations, e.g. updating the packet count more than once for a single input.

\subsection{Avoid packet re-parsing}
Service chain is used to meet the high level performance and security objectives. In some cases, multiple NFs in the service chain extract the same information from the packet header, e.g. re-parsing the same protocol header or reconstructing the same session. NFs must reuse the information parsed or constructed by one instance to avoid resource wastage.

\subsection{Ensure packet ordering}
\label{trojanexample}
Some NFs require ordering across different flows for their processing. For example, the multistep trojan detector described in ~\cite{lorenzos_work} uses across flow state analysis to identify a trojan. The IDS leverages the fact that the particular trojan perform following sequence of steps: (1) opens an SSH connection; (2) downloads an HTML file and a ZIP and EXE file over an FTP connection; (3) generate IRC activity. The order of the steps is relevant, any different order does not indicate the fingerprint of the trojan. Ensuring ordering across flows, when the flows are processed by different instances is hard because synchronizing clock is expensive. A naive approach to ensure ordering across flows would be to use scope-aware partitioning to process all the flows which have ordering requirement on a single instance. However, this limits the ability of the framework to scale. A framework must ensure ordering across the flow, if required.

\subsection{Dynamic service chaining}
Network operators use NFs in service chains to meet high-level policy objectives, such as performance, resource monitoring and security objective. For example, a policy could be that all incoming traffic passes through a Firewall, followed by a caching proxy, and a load balancer. Additionally, a network operator may also want to dynamically add and or remove an NFs from the service chain in response to changes in the network traffic. For example, a deep packet inspection (DPI) engine may need to be added to the chain for further inspection if the firewall detects some malicious activity. Similarly, an NF may be needed to be removed from the chain when it is no longer needed to reduce packet latency and resource wastage.

\subsection{Efficient placement}
The framework must not only reduce cross rack traffic, but also avoid unnecessary usage of switch capacity by efficiently placing the instances in the rack. In addition to this, the instance may have hardware requirements for their operation such as remote memory access (RDMA), encryption engine or hardware accelerator. Prior work \cite{gember2013stratos,E2} has looked at efficient placement, in this paper, we do not focus on efficient placement.



==> paper - Copy/dagapi.tex <==
\section{Framework: Operator View}
\label{sec:api}


In \name, operators define ``logical'' NF chains (such
as~\figref{fig-logical-chain}) using a DAG API. We elide low level
details of the API, such as how policies are specified,
and focus on aspects related to correctness and
performance. Each ``vertex'' of the DAG is an NF and consists of
operator supplied NF code, input/output, configuration, and state
objects. Edges represent the flow of data (packets and/or
contextual output). %%from an upstream vertex to a downstream vertex.


%% Packets flow from the DAG source towards sinks while traversing
%% internal vertices. 
%% Each vertex may: (a) analyze incoming packets; (b)
%% transform packets; (c) generate contextual output (e.g., raise
%% specific events or alarms), and (b) update state objects (more
%% below). Edges represent data flow, and edge annotations reflect
%% aspects of the data flowing between vertices (e.g., the specific set
%% of flows).


%% \textbf{Logical DAG:} The user defines a logical DAG (as shown in line
%% 1 in \figref{fig-dag-code}) with worker instances as vertices. Each
%% worker represents a packet processing unit. The edges in the DAG,
%% represent the flow of packets from one worker to another, along with
%% the output produced by an upstream worker.

\iffalse
\begin{figure}

\begin{lstlisting}[basicstyle=\footnotesize\ttfamily,xleftmargin=2em,numbers=left,breakautoindent=true,columns=fixed,basewidth=0.43em,breaklines=true,language=Java]
logicalDAG dag = new logicalDAG();
vertex vIDS = new vertex(IDS.executor);
vertex vDPI = new vertex(DPI.executor);
vertex vRatelimiter = new vertex(ratelimiter.executor);

edge e1 =  new edge(vIDS.scope());
edge e2 =  new edge(vDPI.scope(), filter());
edge e3 =  new edge(vRateLimiter.scope());
edge e4 =  new edge();

dag.addVertex(vIDS).addVertex(vDPI).addVertex(vRateLimiter);
dag.addEdge(dataSrc.out_port, vIDS.in_port, e1).addEdge(vIDS.out_port1, vDPI.in_port,e2).addEdge(vIDS.out_port2, vRatelimiter.in_port, e3).addEdge(vRateLimiter.out_port, dataSink.in_port, e4);
\end{lstlisting}
\vspace{-1.0em}
  \compactcaption{ DAG specification for the example in
    \figref{fig-dag-logical}.} 
%\vspace{-1em}
  \label{fig-dag-code}
\end{figure}
\fi


\label{vertman}



The \name framework compiles the logical DAG into a physical DAG with
logical vertex mapped to one or more {\em instances}
(\figref{fig-dag-phy}).  For example, the IDS
in~\figref{fig-logical-chain} is mapped to three instances
in~\figref{fig-dag-phy}.  The operator can provide default parallelism
per vertex, or this can be determined at run time using
operator-supplied logic (see below). \name deploys the instances
across a cluster.  Each instance processes a partition of the traffic
input to the logical vertex; \name automatically determines the traffic
split to ensure even load distribution (\secref{s:design}).
%(\secref{vertman}).

The \name framework supports chain elastic scaling and straggler
mitigation. Note that the logic, e.g., when to scale is not our focus;
we are interested in high performance state management and COE during
such actions. Nevertheless, we outline the operator-side view
for completeness: Operators must supply relevant logic for each vertex
(i.e., scaling\footnote{e.g., ``when input traffic volume increased
  by a certain $\theta$''}; identifying
stragglers\footnote{when an instance processing $\theta\%$ slower than
  other instances}). \name executes the logic with input from a
``vertex manager'', a logical entity is responsible for collecting
statistics from each vertex's instances, aggregating them, and
providing them periodically to the logic.

Based on user-supplied logic, \name redirects traffic to (from) scaled up
(down) NF instances or clones of straggler NFs. \name manages
state under such dynamic actions to ensure COE. \name also
ensures system-wide fault tolerance. It automatically recovers from
failures of NFs or of \name framework components while always
preserving COE.
%% Our focus on this paper
%% is on how to do the reallocation and failover correctly and in a
%% high-performance manner, and not on the user-supplied logic.


%% The user can also provide custom implementation of the hints
%% generator.

%% We solve the problems of existing frameworks and network function management platforms by externalizing the internal storage, adding splitter instances in addition to worker instances in the DAG. ~\figref{fig-overview} shows the architecture of our system. Following is an overview of 
%% the key components:

%[basicstyle=\small\ttfamily,xleftmargin=2em,numbers=left,breakautoindent=true,columns=fixed,basewidth=0.43em,breaklines=true,language=Java]

\iffalse
\begin{figure}[!h]
	
	\setstretch{0.9}
	\begin{lstlisting}[     
		language=Java,                  % language code
		basicstyle=\footnotesize,      % font size
		numbers=left,                  % where to put line numbers
		numberstyle=\footnotesize,     % numbers size
		numbersep=-3.5pt,                 % how far the line numbers are from the code
		backgroundcolor=\color{white}, % background color
		showspaces=false,                          % show spaces (with underscores)
		showstringspaces=false,            % underline spaces within strings
		showtabs=false,                            % show tabs using underscores
%		frame=single,                  % adds a frame around the code
		tabsize=3,                     % default tabsize
		breaklines=true,                  % automatic line breaking
		columns=fullflexible,
		breakautoindent=false,
		framerule=1pt,
		xleftmargin=0pt,
		xrightmargin=0pt,
		breakindent=0pt,
		basewidth=0.3em,
		resetmargins=true]
	logicalDAG dag = new logicalDAG();
	vertex vIDS = new vertex(IDS.executor);
	vertex vDPI = new vertex(DPI.executor);
	vertex vRatelimiter = new vertex(ratelimiter.executor);
	
	edge e1 =  new edge(vIDS.scope());
	edge e2 =  new edge(vDPI.scope(), filter());
	edge e3 =  new edge(vRateLimiter.scope());
	edge e4 =  new edge();
	
	dag.addVertex(vIDS).addVertex(vDPI).addVertex(vRateLimiter);
	dag.addEdge(dataSrc.out_port, vIDS.in_port, e1).addEdge(vIDS.out_port1, vDPI.in_port,e2).addEdge(vIDS.out_port2, vRatelimiter.in_port, e3).addEdge(vRateLimiter.out_port, dataSink.in_port, e4);
	\end{lstlisting}
%	\vspace{-1.0em}
	\compactcaption{ DAG specification for the example in
		\figref{fig-dag-logical}.} 
	%\vspace{-1em}
	\label{fig-dag-code}
\end{figure}
\fi
%% Optionally,
                                                                                %% the
%% user can
%% provide hints about the number of tasks executing a vertex when the
%% DAG first executes.

%% The physical DAG also includes special vertices
%% called splitters as shown in \figref{fig-dag-phy}. Each splitter
%% vertex parses input packet headers and distributes the input traffic
%% load among downstream tasks



==> paper - Copy/eval.tex <==
\vspace{-0.1in}
\section{Evaluation}
\label{eval}
\label{s:eval}

 We use two packet traces (Trace\{1,2\}) collected on the link between
 our institution and AWS EC2 for  trace-driven evaluation of our
 prototype. Trace1 has 3.8M packets with 1.7K connections and Trace2
 has 6.4M packets with 199K connections. The median packet sizes are
 368B and 1434B. We conducted all experiments with both traces and
 found the results to be similar; for brevity, we only show results
 from Trace2. We use six CloudLab~\cite{cloudlab} servers each with
 8-core Intel Xeon-D1548 CPUs and a dual-port 10G NIC. One port is
 used to forward traffic, and the other for datastore communication
 and control messages. To process at 10Gbps, each NF instance runs
 multiple processing threads. \name performs scope-aware partitioning
 of input traffic between these threads. Our datastore runs on a
 dedicated server.

%The RTT between any two
%  pairs of servers is 135$\mu$s. 
 

%% \

%% We start with microbenchmarks that evaluate the impact of externalizing internal state (\ref{extern_state}). Next, we show the overhead of maintaining a logical clock (\ref{logical_clock_overhead}), followed by the overhead of logging input packets (\ref{logging_overhead}), and finally the performance of scaling (\ref{}), fault tolerance (\ref{}) and straggler mitigation (\ref{}).
\vspace{-.1in}
\subsection{State Management Performance}
\label{extern_state}

{\bf Externalization:} We study three models which reflect the state
access optimizations discussed in (\secref{storage-sec}): \#1) All
state is externalized and non-blocking operations are used. \#2)
Further, NFs cache relevant state objects. \#3) Further, NFs do not
wait for ACKs of non-blocking operations to state objects; the
framework is responsible for retransmission
(\secref{storage-sec}). \CR{The state objects per NF that benefit from \#2
and \#3 can be inferred from \tabref{ts:iostrategies}	and \tabref{ts:nf-state}; e.g., for NAT,
per-connection port mapping is cached in \#2, and
the two packet counters benefit from non-blocking updates in \#3. We
compare these models with a ``traditional'' NF where all state is
NF-local. We study each NF type in isolation first.}

\begin{figure}[t!]
	\begin{center}
			%\vspace{-1em}
		\includegraphics[width=0.45\textwidth]{figures/latency.pdf}
		%%		\vspace{-0.7em}
		\\
			\vspace{-0.1em}

%	\vspace{-0.2em}
	\compactcaption{5\%ile, 25\%ile, median, 75\%ile and 95\%ile pkt processing times. ({\footnotesize T = Traditional NF, EO = Externalized state operations, C = with caching, NA = without waiting for the ACK}) }
	\label{eval-micro-state-exten}
		%		\label{eval-crossflow}
	\end{center}      
		\vspace{-0.2in}  
\end{figure}

%\begin{figure*}[t]
%	\centering
%	\subfloat[][NAT]{%
%		\label{}%
%		\includegraphics[scale=0.40]{figures/nat_micro.pdf}%
%	}
%	\hspace{0em}%\hfill
%	\subfloat[][Port Scan detector]{%
%		\label{fig-ft-naive-reproc} 
%		\includegraphics[scale=0.40]{figures/trw_micro.pdf}%
%	}
%	\hspace{0em}%\hfill
%	\subfloat[][Trojan detector]{%
%		\label{} 
%		\includegraphics[scale=0.40]{figures/ids_micro.pdf}%
%	}
%	\hspace{0em}%\hfill
%	\subfloat[][Load Balancer]{%
%		\label{} 
%		\includegraphics[scale=0.40]{figures/lb_micro.pdf}%
%	}\\
%
%\end{figure*}

~\figref{eval-micro-state-exten} shows the per packet
processing times.
%% \footnote{Time between the framework receiving a packet and
%%   the NF finishing processing.}. 
The median times for traditional NAT and load balancer are 2.07$\mu$s
and 2.25$\mu$s, respectively. In model \#1, this increases by 190.67$\mu$s
and 109.87$\mu$s, respectively, with network RTT contributing to most of
this (e.g., NAT needs three RTTs on average per packet: one for
reading the port mapping and other two for updating the two
counters). We don't see a noticeable impact for scan and Trojan
detectors (they don't update state on every packet).

Relative to \#1, caching (\#2) further lowers median processing times
by 111.98$\mu$s and 55.94$\mu$s for NAT\footnote{NAT needs 2 RTTs to
  update counters as port mapping is cached.} and load
balancer. For portscan and Trojan detector, reduces it by 0.54$\mu$s and 0.1$\mu$s (overhead becomes {\bf+0.1$\mu$s} as compared to traditional NFs) as \name caches the cross-flow state. Later, we evaluate the benefits of cross-flow caching in detail. Finally, \#3 results in median packet processing times of {\bf 2.61$\mu$s} for NAT (which now needs 0 RTTs on average)
and {\bf 2.27$\mu$s} for load balancer. These represent small
overheads compared to traditional NFs: {\bf +0.54$\mu$s} for NAT, and
{\bf +0.02$\mu$s} for the load balancer (at the median). Note that for portscan and Trojan detector the performance of \#3 is comparable to \#2 as they don't have any blocking operations.

We constructed a simple chain consisting of one instance each of NAT,
portscan detector and load balancer in sequence, and the Trojan
detector operating off-path attached to the NAT. With model \#3, the
median end-to-end overhead was {\bf 11.3$\mu$sec} compared to using
traditional NFs.



%% median latency increases {\bf +0.54$\mu$s} (likewise, 75\%ile
%% increases 1.22$\mu$s); load balancer's median latency increases  (likewise, 75\%ile increases 6.15$\mu$s).



%% Not waiting for the ACKs of update operations further reduce the latency by 1 RTT.
%% From \figref{eval-NAT-latency}, we see that the network contributes
%% around 122$\mu$s (2*RTT) when NAT externalizes all of its internal
%% state. Reducing the network latency can significantly improve the
%% performance. The packet processing latency is reduced by 1 RTT when
%% \aditya{the rest of this sentence does not parse:} the NAT
%% caches the port mapping and does read it on every packet from the datastore. Not waiting for the ACKs of update operations further reduce the latency by 1 RTT.


%% \begin{figure}[h!]
%% 	%	\vspace{-1em}
%% 	\begin{center}
%% 		\includegraphics[width=0.50\textwidth]{figures/nat_micro_network}
%% 	\begin{scriptsize}
%% 		T = Traditional NF, EO = Externalized state operations, C = with caching, NA = without waiting for the ACK 
%% 	\end{scriptsize}
%% 		\compactcaption{Average packet processing time of NAT.}
		
%% 		\label{eval-NAT-latency}
%% 	\end{center}        
%% \end{figure}

{\bf Operation offloading:} We compare \name's operation offloading
against a naive approach where an NF first reads state from
the datastore, updates it, and then writes it back. We turn off
caching optimizations. We now use two NAT instances updating shared state
(available ports and counters). We find that the median packet
processing latency of the naive approach is {\bf 2.17X} worse
(64.6$\mu$s vs 29.7$\mu$s), because it not only requires 2 RTTs to
update state (one for reading the state and the other for writing it
back), but it may also have NFs wait to acquire locks.
%% In \name, state update
%% happens in a single RTT and locks are not needed.
\name's aggregate
throughput across the two instances is $>$2X better.

{\bf Cross-flow state caching:} To show the performance of our
cross-flow state caching schemes (\tabref{ts:iostrategies}; Col 5), we
run the following experiment: we start with a single portscan
detector. After it has processed around 212K packets, we add a second
instance and split traffic such that for particular hosts, captured by
the set $\mathcal{H}$, processing happens at both instances. At around
213K packets, we revert to using a single instance for all
processing. \figref{eval-crossflow} shows the benefits of
caching the shared state. At 212K packets, when the second instance is
added, the upstream splitter signals the original instance to flush
shared state corresponding to hosts $\in \mathcal{H}$
(\tabref{ts:nf-state}). From this point on, both instances make
blocking state update operations to update the likelihood of hosts
$\in \mathcal{H}$ being malicious on every successful/unsuccessful
connection initiation. Thus, we see an increase in per packet
processing latency for every SYN-ACK/RST packet. At packet number
213K, all processing for $\mathcal{H}$ happens at a single instance
which can start caching state again. Thus, the processing latency for
SYN-ACK/RST packets drops again, because now state update
operations are applied locally and updates are flushed in a
non-blocking fashion to the store.

\begin{figure}[t!]
	\begin{center}
				%\vspace{-1em}
		\includegraphics[width=0.47\textwidth]{figures/caching-crossflow.pdf}
		%%		\vspace{-0.7em}
		\\
		%%	\vspace{-0.1em}
		\compactcaption{Per packet processing latency with cross-flow state caching}
		\label{eval-crossflow}
	\end{center}      
		\vspace{-1em}  
\end{figure}



{\bf Throughput:} We measure degradation in per NF throughput for
models \#1 and \#3 above compared to traditional
NFs. \figref{eval-ft-throughput} shows that the max. per NF
throughput for traditional NFs is around 9.5Gbps. Under model \#1,
load balancer and NAT throughput drops to 0.5Gbps. The former needs
to update a byte counter (which takes 1 RTT) on every packet;
likewise, the NAT needs three RTTs per packet. The port scan and Trojan
detectors do not experience throughput degradation because they don't
update state on every packet. Model \#3 increases throughput to
9.43Gbps, matching traditional load balancer and NAT. We repeated our
experiment with the aforementioned single-instance NF chain and
observed similar maximal performance (9.25Gbps with both \name and
traditional NFs) in Model \#3.

\begin{figure}[t!]
	\begin{center}
		%%		\vspace{-1em}
		\includegraphics[width=0.45\textwidth]{figures/throughput.pdf}
		%%		\vspace{-0.7em}
		\\
		%%	\vspace{-0.1em}
		\compactcaption{Per instance throughput. (T = Traditional NF, EO = Externalized state operations, C = with caching, NA = without waiting for the ACK)}
		\label{eval-ft-throughput}
	\end{center}      
	\vspace{-1em}  
\end{figure}

{\bf Datastore performance} We benchmarked the datastore using the
workload imposed by our state operations. \CR{We used 128bits key and  64bits value to benchmark the datastore. The datastore was running four threads. Each thread handled 100k unique entries. As discussed in \secref{storage-sec}, state is not shared between these threads.} We found that a single instance of our datastore supports {\bf $\sim$5.1M} ops/s (increment
at 5.1M ops/s, get at 5.2M ops/s, set at 5.1M ops/s;
~\tabref{t:operations}). The datastore can be easily scaled to support a greater
rate of operations by simply adding multiple instances; each
state object is stored at exactly one store node and hence no cross-store node
coordination is needed.

\subsection{Metadata Overhead}

{\bf Clocks:} The root writes packet clocks to the
datastore for fault tolerance. This adds a 29$\mu$s
latency per packet (dominated by RTT). We optimize further by writing
the clock to the store after every n$^{th}$ packet.\footnote{After a
  crash, this may lead the root to assign to a packet an already
  assigned clock value. To overcome this issue, the root starts
  with {\em n + last update} so that clock values
  assigned to packets represent their arrival order.}  The average
overhead per packet reduces to 3.5$\mu$s and 0.4$\mu$s for
$n=10, 100$.
	
	%% \figref{eval-clock} shows the overhead
	%% of this.  Again, a significant part (97.5$\%$) of this overhead comes
	%% from the network. 
	
	%% \label{logical_clock_overhead}
	%% \begin{figure}[h!]
	%% 	\begin{center}
	%% 		\includegraphics[width=0.50\textwidth]{figures/clock.pdf}
	%% 		\vspace{-2em}
	%% 		\compactcaption{Average per packet overhead of updating the logical clock.}
	%% 		\label{eval-clock}
	%% 	\end{center}        
	%% \end{figure}
	
	\label{logging_overhead}
	{\bf Packet logging:} We evaluated two models of logging: 1)
        locally at the root, 2) in the datastore.  The former
        offers better performance, adding 1$\mu$s latency per packet,
        whereas the latter adds 34.2$\mu$s but is more fault tolerant
        (for simultaneous root and NF failures).  We also studied the
        overhead imposed by the framework logging clocks and
        operations at NFs, the datastore logging clocks and state, and
        the XOR-ing of identifiers (\secref{s:ft-in}); the 
        performance impact for our chain (latency and throughput
        overhead) was negligible ($<1$\%).
        
	%%     comparing with a remote DB?} The first model has a negligible
	%%   impact of 1.81$\mu$s (shown in \figref{eval-logging}) in the per
	%%   packet latency. The second model adds around 71.5$\mu$s to per
	%%   packet latency. However most of it comes from the network
	%%   latency. \aditya{logging needs a complete rewrite}
	
	
	%% \begin{figure}[h!]
	%% 	\begin{center}
	%% 		\includegraphics[width=0.50\textwidth]{figures/logging.pdf}
	%% 		\vspace{-2em}
	%% 		\compactcaption{Per packet overhead of logging packets.}
	%% 		\label{eval-logging}
	%% 	\end{center}        
	%% \end{figure}

\JK{{\bf XOR check and delete request:} (\secref{s:ft-in}) XOR checks of bit vectors are performed asynchronously in the background and do not introduce any 
latency overhead.  However, ensuring the successful delivery of ``delete'' request to root before forwarding the packet 
introduces a median latency overhead of 7.9$\mu$sec. Asynchronous ``delete'' request operation eliminates this overhead but failure of the last NF in a chain may result in duplicate packets at the receiver end host.

}
\subsection{Correctness Requirements: R1--R6}
\label{statemanagement-eval}

{\bf R1: State availability:} Using our NAT, we compare
FTMB's~\cite{ftmb} checkpointing approach with \name writing all state
to a store.  We could not obtain access to FTMB's code; thus, we
emulate its checkpointing overhead using a queuing delay of 5000$\mu$s
after every 200ms (from Figure 6 in \cite{ftmb}).
\figref{eval-ft} (with 50\% load level) shows that checkpointing in
FTMB has a significant impact: the 75th\%-ile latency is 25.5$\mu$sec
-- which is {\bf 6X} worse than that under \name (median is 2.7X
worse).  FTMB's checkpointing causes incoming packets to be
buffered. Because of externalization in \name, there is no need for such
checkpointing.
%% , and hence this latency in \name is just
%% 4.28$\mu$sec. Median latency is 4.93$\mu$sec in FTMB vs 1.82$\mu$sec
%% in \name.
Also, FTMB does not support recovery of the packet
logger~\cite{ftmb}. \name intrinsically supports this
(\secref{s:ft-in}), and we evaluate it in \secref{s:ft-eval}.

{\bf R2: Cross-instance state transfers:} We elastically scale up NAT as follows: We replay our trace for 30s through a single instance;
midway through replay, we reallocate 4000 flows to a new instance,
forcing a move of the state corresponding to these flows.  We compare
\name with OpenNF's loss-free move; recall that \name provides both
loss-freeness and order preservation.  \name's move operation takes
97$\%$ {\bf or 35X } less time (0.071ms vs 2.5ms), because, unlike
OpenNF, \name does not need to transfer state. It notifies the
datastore manager to update the relevant instance$\_$IDs.  However,
when instances are caching state, they are required to flush cached
state operations before updating instance$\_$IDs. Even then, \name
is 89\% better because it {\em flushes only operations}. %% Finally, unlike
%% \name, OpenNF cannot prevent packet reordering at downstream NFs
%% due to state transfer at upstream NFs (\secref{g:scaling}).

%% \begin{figure}[h!]
%% 	\begin{center}
%% 		\includegraphics[width=0.50\textwidth]{figures/state_scaling.pdf}
%% 		\vspace{-2em}
%% 		\compactcaption{Average per flow transfer transfer time.}
%% 		\label{eval-scaling-transfer}
%% 	\end{center}        
%% \end{figure}

{\bf R3: Cross-instance state sharing:} We compare \name against
OpenNF w.r.t. the performance of strongly consistent shared state
updates across NAT instances, i.e., updates are serialized according
to some global order. \figref{eval-scaling} (with 50\% load level)
shows that \name's median per-packet latency is 99\% lower than
OpenNF's (1.8$\mu$s vs 0.166ms). The OpenNF
controller receives all packets from NFs; each is forwarded to every
instance; the next packet is released only after all instances
ACK. \name's store simply serializes all instances' offloaded
operations.



%% reduces the 50 $\%$-ile per packet processing time from .8msec to
%% 6.8$\mu$s. The gain in the performance of \name comes from the
%% fact that it eliminates the synchronization overhead of state sharing
%% by offloading state update operations to the datastore
%% manager. Whereas OpenNF requires strong synchronization for state
%% sharing. The central controller in OpenNF is required to read the
%% state from one instance and copy it to all the other instances in a
%% pairwise fashion.


%% ~\figref{pkt-scaling} shows the per packet processing latency after
%% flows are moved across two NAT instances. As there is no cached state,
%% the first ~15k packets experience relatively high processing time. The
%% minimum packet processing time is also higher for first 20k
%% packets. This is due to buffering of packets when the new instance is
%% waiting for the old instance to flush the cached state.}

%%  \begin{figure}[h!]
%% 	\begin{center}
%% 		\includegraphics[width=0.50\textwidth]{figures/scaling_pppt.pdf}
%% 		\vspace{-2.5em}
%% 		\caption{Per packet processing time.}
%% 		\label{pkt-scaling}
%% 	\end{center}        
%% \end{figure}

\begin{figure}[!t]
	%\vspace{-0.1in}
	\begin{minipage}[t]{0.4\linewidth}
		\centering
		\includegraphics[width=1\textwidth]{figures/state_sharing.pdf}
		\caption{State sharing.}
		\label{eval-scaling}
	\end{minipage}
	\hspace{0.1cm}
	\begin{minipage}[t]{0.4\linewidth} 
		\centering
		\includegraphics[width=1\textwidth]{figures/ftmb.pdf}
		\caption{Fault recovery.}
		\label{eval-ft}
	\end{minipage}        
\vspace{-0.12in}
\end{figure}  


%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=0.48\textwidth]{figures/ftmb.pdf}
%		\vspace{-2.5em}
%		\compactcaption{Per packet processing time with fault tolerance.}
%		\label{eval-ft}
%	\end{center}        
%	\vspace{-1em}
%\end{figure}

%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=0.24\textwidth]{figures/state_sharing.pdf}
%		\vspace{-2.5em}
%		\compactcaption{Per packet processing time with state sharing.}
%		\label{eval-scaling}
%	\end{center}        
%\end{figure}

%% \subsection{R4 \& R5: Chain-wide ordering \& duplicate suppression}

%\input{tables/duplicate_supression}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{0.5em}
\small
\begin{tabular}{l||cc}
& 30$\%$load& 50$\%$load\\

\hline
\hline
			
Duplicate packets & 13768 & 34351\\
Duplicate state updates & 233 & 545 \\

\end{tabular}
\compactcaption{Duplicate packet and state update at the downstream portscan detector without duplicate suppression.\label{ts:duplicate1}
}
%\end{scriptsize}
%\vspace{-1em}
\vspace{-0.1in}
\end{table}

{\bf R4: Chain-wide ordering:} We revisit the chain
in~\figref{fig-example-trojan}. Each scrubber instance processes
either FTP, SSH, or IRC flows. To measure the accuracy of the Trojan
detector, we added the signature of a Trojan at 11 different points in
our trace. We use three different workloads with varying
upstream NF processing speed: W1) One of the upstream NFs
adds a random delay between 50-100$\mu$s to each packet. W2)
Two of the upstreams add the random delay. W3) All three add random
delays. We observed that \name's use of chain-wide logical clocks
helps the Trojan detector identify {\bf all 11 signatures}.  We
compare against OpenNF which does not offer any chain-wide guarantees;
we find that {\bf OpenNF misses 7, 10, and 11 signatures} across
W1--W3.

{\bf R5: Duplicate suppression:} Here, we emulated a straggler NAT by
adding a random per packet delay between between 3-10$\mu$s. A portscan detector is immediately downstream from the NAT. \name launches a
clone NAT instance according to \secref{straggler}. We vary the input
traffic load.  Table~\ref{ts:duplicate1} shows the number of duplicate
packets generated by the NAT instances under different loads, as well
as the number of duplicate state updates at the portscan detector --
which happen whenever a duplicate packet triggers the scan detector to
{\em spuriously} log a connection setup/teardown attempt.  Duplicate
updates create both false positives/negatives and their incidence
worsens with load. No existing framework can detect such
duplicate updates; \name simply suppresses them.
%% that arise due to upstream
%% NF actions.



%\subsection{R6: Fault Tolerance}
\label{s:ft-eval}

{\bf R6: Fault Tolerance:} We study  \name failure recovery.

{\em NF Failure:} We fail a single NAT instance and measure the
recovery and per packet processing times. Our NAT performs
non-blocking updates without waiting for the framework ACK; here, we
use the 32bit vector (\secref{faulttolerance}) to enable recovery of
packets whose non-blocked operations are not yet committed to the store. To focus
on \name's state recovery, we assume the failover container is
launched immediately. \figref{eval-ft-reply} shows the average
processing time of packets that arrive at the new instance at two
different loads. The average is calculated over 500$\mu$s
windows. Latency during recovery spikes to over 4ms, but it only takes
{\bf 4.5ms} and {\bf 5.6ms} at 30\% and 50\% loads,
respectively, for it to return to normal.

%% In ~\secref{statemanagement-eval}, we showed that \name can recover from NF instance failures in less than a millisecond. In this section we evaluate the recovery time and impact of failure of storage and root splitter on the per packet processing latency.

{\em Root failure:} Recovering a root requires just
reading the last updated logical clock from the datastore and
 flow mapping from downstream NFs. This takes $<41.2\mu$s.


{\em Datastore instance failure:} Recovering a datastore instance
failure requires reading per-flow state from NFs using it, and
replaying update operations to rebuild shared state. Reading the
latest values of per-flow state is fast. Recovering shared state
however is more time-consuming.  ~\figref{eval-ft-chkpt} shows the
time to rebuild shared state with 5 and 10 NAT instances updating the
same state objects at a single store instance. We replayed the state
update operation logs generated by these instances. The instances were
processing 9.4Gbps of traffic; periodic checkpoints occurred at
intervals of 30ms, 75ms, and 150ms. The recovery time is {\bf $\le$
  388.2ms} for 10 NATs with checkpoints at 150ms intervals. In other
words, a storage instance can be quickly recovered.
%%  In our experiments we are using a single Redis
%% server based datastore. As with I/O (\secref{extern_state}), recovery
%% time can be decreased by using multiple servers for the datastore.

\begin{figure}[!t]
		%\vspace{-0.1in}
		\hspace{-0.4cm}%
	\begin{minipage}[b]{0.50\linewidth}
		\centering
		\includegraphics[valign=T,width=1.05\textwidth]{figures/ft_replay.pdf}
		\vspace{-1.0em}
		\caption{Packet proc time.}
		\label{eval-ft-reply}
	\end{minipage}%
	%\hspace{0.38cm}%
	\hfill
	\begin{minipage}[b]{0.43\linewidth} %
		\centering
		\includegraphics[valign=T, width=1.05\textwidth]{figures/storage_chkpt.pdf}
		\vspace{0.05in}

		\caption{Store recovery.}
		\label{eval-ft-chkpt}
	\end{minipage}        
	\vspace{-0.25in}
\end{figure}  

%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=0.47\textwidth]{figures/ft_replay.pdf}
%		\vspace{-1.2em}
%		\compactcaption{Avg.  per pkt processing time after a failure.}
%		\label{eval-ft-reply}
%	\end{center}        
%\end{figure}

%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=0.48\textwidth]{figures/storage_chkpt.pdf}
%		\vspace{-2.5em}
%		\compactcaption{State update operation replay overhead.}
%		\label{eval-ft-chkpt}
%	\end{center}        
%\end{figure}

%% We ran the same experiment as describe in ~\secref{statemanagement-eval}

%To measure the impact of datastore failure on per
%packet processing time, we study a setup with periodic datastore
%checkpoints at 30ms intervals and 20 NAT instances using the
%store. ~\figref{eval-ft-redis-replay} shows the average per packet
%processing time upon failure, where average is calculated over a window
%of 400$\mu$s. It takes {\bf 420ms} and {\bf 455ms} for average per
%packet processing time to return to normal at 50\% and 75\% load
%level, resply. During replay of state update operations, packets
%can not be processed and must be buffered.  When processing resumes,
%the per packet processing time increases for a short duration
%because of the buffering.
%
%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=0.47\textwidth]{figures/ft_redis_replay.pdf}
%		\vspace{-1.3em}
%		\compactcaption{Average per pkt processing time after a failure.}
%		\label{eval-ft-redis-replay}
%	\end{center}        
%\end{figure}


%% In summary, \name offers better performing, more general state
%% management than state of the art techniques and can ensure chain-wide
%% guarantees at a most per-packet latency overhead.


%% \figref{eval-ordering} However, the NF without any chain wide order guarantees
%% missed 63-100$\%$ of the signatures (shown in \figref{eval-ordering})
%% \begin{figure}[h!]
%% 	\begin{center}
%% 		\includegraphics[width=0.50\textwidth]{figures/chain_ordering.pdf}
%% 		\vspace{-2em}
%% 		\compactcaption{Alarms missed by the Trojan detector w/o chain wide order guarantees.}
%% 		\label{eval-ordering}
%% 	\end{center}        
%% \end{figure}

%% {\bf Evaluation summary:} To summarize, our trace-based evaluation
%% shows the following key points: (1) \name's architecture and
%% associated optimizations for handling externalized state
%% result in low latency overhead; (2) \name's overall architecture
%% offers imposes low throughput overhead as well. (3) \name's state
%% management offers much better performance than state-of-the-art, and
%% ensures fault tolerance at much lower overhead; (4) \name supports
%% novel safety properties, such as duplicate suppression and chain-wide
%% ordering, which existing systems lack causing them to generate
%% spurious alerts and miss identifying attacks.



==> paper - Copy/faulttolerance.tex <==


\subsection{R6: Safe Fault Recovery}
\label{faulttolerance}
\label{s:ft-in}

%\begin{figure*}[t]
%       \centering
%       \subfloat[][Normal processing without any failure]{%
%               \label{fig-ft-normal}%
%               \includegraphics[scale=0.60]{figures/ft_normal.pdf}%
%       }
%       \hspace{0em}%\hfill
%       \subfloat[][Naive reprocessing]{%
%                \label{fig-ft-naive-reproc} 
%               \includegraphics[scale=0.60]{figures/ft_nv_reproc.pdf}%
%       }
%      \hspace{0em}%\hfill
%       \subfloat[][Reprocessing with emulation]{%
%                \label{fig-ft-reproc} 
%               \includegraphics[scale=0.60]{figures/ft_reproc.pdf}%
%       }
%       %\vspace{-0.8em} 
%       \compactcaption{Reprocessing of packet after a
%         failure or cloning (both are simular). Figure \(a\) \& \(b\)
%         illustrate the problem.}
%       \label{fig-ft}
%\end{figure*}


\JK{ Our description of R6 in \secref{s:mot} focused on NF failures;
  however, since \name introduces framework components, we generalize
  R6 to cover other failures as well. Specifically, we require the
  following general guarantee:

{\bf Safe recovery Guarantee:} {\em When an NF instance or a framework component fails and a recovery occurs, we must ensure that the state at each NF in the chain has the same value as under no failure.}


%% {\bf Failure Model:}
We assume the standard fail-stop model,  that a machine/node can crash at any time and that the other machines/nodes in the system can immediately detect the failure.

First, we show how \name leverages metadata to handle the failure of individual components. Then, we discuss scenarios involving simultaneous failure of multiple components.
}
  
{\bf NF Failover:} When an NF fails, a failover instance takes over
the failed instance's processing. The datastore manager associates the
failover instance's ID with relevant state. Packet replay brings state
up-to-speed (from updates due to in-transit packets). Similar to
cloning (\secref{stragglers}), we suppress duplicate state
updates and upstream processing.

Since ``delete'' requests are generated after the last NF is done
processing a packet, failure of such an NF needs special handling:
consider such an instance T failing after generating an output packet
for some input packet P, but before the framework sends a ``delete''
request for P.  When P is replayed, T's failover instance produces
output again, resulting in duplicate packets at the receiving end
host. To prevent this, for the last NF in the chain, our framework
sends the ``delete'' request for P {\em before} the NF generates the
output packet. If the NF fails before the ``delete'' request, then P
will be replayed, but this does not result in duplicate downstream
processing since the NF did not generate output.  If the NF fails
after the ``delete'' request but before generating output, then P is
not replayed, and hence the end host will not receive any output
packet corresponding to P. \CR{To the host, this will appear as a packet being dropped by the network, causing P to be retransmitted from the source and resulting in
correct overall behavior.} In \secref{secproof:nfrecovery}, we show that using this
  protocol an NF instance recovers with state similar to that under
  no failure.

\begin{figure}[tb]
	\vspace{-.1in}
	\centering
		\includegraphics[scale=0.68]{figures/nonblocking.pdf}%
	        %\vspace{-0.8em}
                \compactcaption{Recovery under
                non-blocking operations. Consider a packet $P^i$ which
                is processed by $NF_N$, followed by $NF_M$, the last NF in the
                chain. $NF_N$ and $NF_M$ update objects $obj_Y$ and $obj_Z$, respectively.}
                
	\label{fig-nonblocking-ft}
	\vspace{-0.08in}
\end{figure}


{\bf Non-blocking operations:} Non-blocking updates, where NF
instances don't wait for ACKs, instead relying on the framework to
handle reliable delivery, can introduce the following failure mode: a
instance may fail after issuing state update but before the
update is committed and an ACK was received. In such cases, to ensure
R6, we need that {\em the framework must re-execute the incomplete
  update operation.}

Suppose an instance $N$ fails after processing packet $P_i$ ($i$ is the
logical clock) but before the corresponding state update operation
$U_{N,obj}^i$ ($obj$ is the state object ID) completes. $P_i$ may have
induced such operations at a subset of NF instances $\{N\}$ along the
chain.  A natural idea to ensure the above property is to replay
packets from the root to reproduce $U_{N,obj}^i$ at various $N$'s. For
this, however, $P_i$ must be logged and should not have been
deleted. If $P_i$ is deleted it can't be replayed.

We need to ensure $P_i$ continues to be logged as long as there is
some $N$ for which $U_{N,obj}^i$ is not committed. Our approach for
this is shown in~\figref{fig-nonblocking-ft}: \circled{1} Each packet carries
a 32-bit vector $v_i$ (object ID and instance ID; 16b each) that is
initialized to zero. Each NF instance where processing the packet
resulted in a state update XORs the concatenation of its ID and the
corresponding state objects' IDs into the bit vector.  \circled{2} When
committing a given NF's state update, the state store signals to the
root the clock value of the packet that induced the update as
well as the concatenated IDs. \circled{3} The last instance sends the final
vector along with its ``delete'' request to the root. \circled{4} When a delete
request and the final vector are received, the root XORs the
concatenated IDs with the concatenated IDs reported by each signal
from the state store in step 2. If the result is zero, this implies
that updates induced by the packet at all NF instances $\{N\}$ were
committed to the store; the root then proceeds to delete the
packet from the log. Otherwise, the packet updated state at some NF,
but the NF has not yet reported that the state was committed; here,
the root does not delete the packet.


%%  To make the
%% framework fully fault tolerant, other components, storage system and
%% root splitters are also needed to be fault tolerant. Their recovery
%% must be fast to avoid causing any degradation in per packet processing
%% latency.

{\bf Root:} To ensure R6 under root failover, we need that a new root
must start with the logical clock value and current flow allocation at
the time of root failure. This is so that the new root processes
subsequent packets correctly. To ensure this, the failover root reads
the last updated value of the logical clock from the datastore, and
retrieves how to partition traffic by querying downstream instances'
flow allocation. The framework buffers incoming packets during root
recovery. \JK{We prove this approach ensures recovery with a state similar to that under no failure in   \secref{secproof:rootrecovery}.}


{\bf Datastore instance:} Recall that different NFs can store their
states in different storage instances (\secref{storage-sec}). This
ensures that store failures impact availability of only a portion of
the overall state being tracked. Now, to ensure R6 under the failure
of a datastore instance, we need that the recovered state in the new
store instance must represent the value which would have resulted if
there was no failure. The recovered state must also be consistent with
the NF instances' view of packet processing thus far (i.e., until
failure).

To support this property we distinguish between per-flow and shared
state. For the former, we leverage the insight that all the NFs
already maintain an updated cached copy of per-flow state. If a
datastore instance fails, we can simply query the last updated value of the
cached per-flow state from all NF instances that were using the store.

%% As only one NF updates the
%% per-flow state, it does not require any synchronization.

\JK{Recovering shared state is nuanced. For this, we use
checkpointing with write-ahead logging~\cite{wal}. The datastore periodically checkpoints
shared state along with the metadata, ``$TS$'', which is the set of
logical clocks of the packets corresponding to the last state
operation executed by the store on behalf of each NF instance. Each
instance locally writes shared-state update operations in a write-ahead log}. Say the latest checkpoint was at time $t$ and failure
happens at $t + \delta$. A failover datastore instance boots with
state from the checkpoint at $t$. This state now needs to be ``rolled
forward'' to $t+\delta$ and made consistent with the NF instances'
view of packet processing at $t+\delta$. Two cases arise:

(Case 1) If NF instances that were using the store instance don't read
shared state in the $\delta$ time interval, then to recover shared
state, the framework re-executes state update operations from the local write-ahead log on behalf of each NF, starting from the logical clocks
included in the metadata $TS$ in the checkpoint. Recall that in our
design the store applies updates in the background, and this update
order is unknown to NF instances. Thus, our approach ensures that the
state updates upon re-execution match that produced by a {\em
  plausible} sequence of updates that the store may have enforced
prior to failure. This consistency property suffices because, in
Case 1, NFs are not reading shared state in the $\delta$ interval.

\begin{figure}[]
	\begin{center}
		\includegraphics[width=0.42\textwidth]{figures/dsfailure.pdf}
                \compactcaption{Recovering shared state at the
                  datastore. $I^k$ are instances.
                  $U^{logical\_clock}$ and $R^{logical\_clock}$
                  represent ``update'' and ``read''.}
		\label{fig-dsfailure}
	\end{center}  
	    \vspace{-1.2em}      
\end{figure}

(Case 2) Say an NF instance issues a read between $t$ and $t +
\delta$; e.g., $I^3$ in \figref{fig-dsfailure} issues
$R^{18}$. Following the above approach may lead to an order of
re-execution such that the actual state $I^3$ read in $R^{18}$ is
different from the state in the store after recovery. \JK{To ensure that
the store's state is consistent with all $I^k$'s current view, the
framework must re-execute operations in such an order that the
datastore would have produced the same value for each read in $[t,
  t+\delta]$.}

To ensure this, on every read operation, the datastore returns $TS$
along with the latest value of the shared state (e.g., $TS^{19}$ is
returned with $I^4$'s $R^{19}$). The instance then logs the value of
the shared state along with the corresponding $TS$.  Re-execution upon
failure then needs to select, among all $TS$'s at different instances,
the one corresponding to the most recent read from the store prior to
the crash (i.e., $TS^{18}$, since $R^{18}$ in the most recent read;
most recent clock does not correspond to most recent read). How
selection is done is explained shortly; but note that when the
framework re-executes updates starting from the clock values indicated
by this selected $TS$ that would bring the store in sync with all
NFs. In our example, $TS^{18}$ is the selected $TS$; we
initialize the store state with the value in the corresponding read
($R^{18}$).  From the write-ahead log of each NF, the framework re-executes
update operations that come after their corresponding logical clocks
in $TS^{18}$. At instance $I^1$, this is the update after $U^{15}$,
i.e., $U^{35}$. At  $I^3$ and $I^4$ these are $U^{23}$ and
$U^{32}$, respectively. Shared state is now in sync with all NFs.

%% \footnote{ The highest logical
%%   value might not always be the most latest value. e.g.  For $I^1$,
%%   the logical clock value 20 appears before 15. This happens when
%%   packets from two different flows, coming from two different upstream
%%   instances, gets reordered.  }

$TS$ selection works as follows: first we form a set of all the $TS$'s
at each instance, i.e., $Set = \{TS^{18},TS^{19},TS^{27}\}$. Since the
log of operations at an instance follows a strict clock order we
traverse it in the reverse order to find the latest update operation
whose corresponding logical clock value is in $Set$.  For example, if
we traverse the log of $I^1$, we find that the logical clock of
$U^{15}$ exists in $Set$. After identifying such a logical clock
value, we remove all the entries from $Set$ which do not contain the
particular logical clock value (such $TS$s cannot have the most recent
read); e.g., we remove $TS^{19}$ as it does not contain logical clock
$15$. Similarly, we remove $TS^{27}$, after traversing $I^2$'s
log. Upon doing this for all instances we end up selecting $TS^{18}$
for recovery. In \secref{secproof:storerecovery}, we prove that using this
protocol the store recovers with state similar to that under no failure.

%% , as well as the mostly recently read value of
%% the shared state.

%% replayed to recover the shared state. To reduce the recovery time, the
%% shared state is periodically checkpointed along with some
%% metadata. This metadata includes the logical clock value of the packet
%% corresponding to last operation executed on the shared state on behalf
%% of each task. The logical clock is later use to determine the starting
%% point in log of the state update operations.  If a task has read the
%% shared state value, we want to execute the operations in such an order
%% that it produces the same value for the read operation. This requires
%% ordering of state update operations across tasks. To avoid maintaining
%% this order, we leverage the insight that the execution order of these
%% state update operations only matters till the last read state
%% operation. In addition to logging the state update operations, we also
%% log the last read value for each state object along with its metadata
%% on each task. This metadata is sent by the datastore manager and it
%% contains the logical clock value of the packet corresponding to last

%%This helps to ensure that a failed datastore instance is safely recovered.

{\bf Correlated failures:} Using the above approaches, \name can also
handle correlated failures (\tabref{ts:mutliplefailures}) of multiple
NF instances, root, and storage instances. However, \name
cannot withstand correlated failure of a store instance with any other
component that has stored its state in that particular
instance. Replication of store instances can help recover from such
correlated failures, but that comes at the cost of increasing the per
packet processing latency.
%% summarizes the
%% simultaneous failures which our framework can handle.

\input{tables/multifailures}



%% {\bf Exactly-once processing:} 



==> paper - Copy/implementation.tex <==
\vspace*{-0.1in}
\section{Implementation}
Our prototype consists of an execution framework and a datastore,
implemented in C++. NFs runs in LXC containers~\cite{lxc} as 
multithreaded processes. NFs are implemented using our \name library
that provides support for input message queues, client side datastore
handling, retransmissions of un-ACK'd state updates
(\secref{g:rexmit}), statistics monitoring and state handling. Packet
reception, transmission, processing and datastore connection
are handled by different threads.

For low latency, we leverage Mellanox messaging accelerator
(VMA)~\cite{vma} which enables user-space networking with kernel
bypass similar to DPDK~\cite{dpdk}. In addition to this, VMA also
supports TCP/UDP/IP networking protocols and does not require any
application modification. Even though we use VMA, we expect similar
performance with other standard kernel bypass techniques.
Protobuf-c~\cite{protobuf} is used to encode and decode messages
between a NF instance and the datastore. Each NF instance is
configured to connect to a ``framework manager'' to receive information
about it's downstream instances (to which it connects via tunnels),
datastore instances and other control information.

The framework manager can dynamically change the NF chain by
instantiating new types of NFs or NF instances and updating
partitioning information in upstream splitters\footnote{based on statistics from vertex managers}. Our datastore
implements an in-memory key-value store and supports the operations
in~\tabref{t:operations}. We reimplemented four NFs atop
\name. Table~\ref{ts:nf-state} shows their state objects, along with
the state's scope and access patterns.


\begin{table}[]
	\centering
    \scriptsize
	\begin{tabular}{p{0.8cm}||p{2.9cm}|p{3.65cm}}

		{\bf NF} & {\bf Description of state object} & {\bf Scope; access pattern} \\ 
		\hline 
		\hline
		\multirow{2}{*}{}
		& Available ports& Cross-flow; write/read often \\ \cline{2-3} 
		NAT& Total TCP packets & Cross-flow; write mostly, read rarely \\ \cline{2-3} 
		& Total packets& Cross-flow; write mostly, read rarely \\ \cline{2-3} 
		& Per conn. port mapping&  Per-flow; write rarely, read mostly\\ 
		\hline 
		\hline
 		\multirow{2}{*}{}Trojan detector& Arrival time of IRC, FTP and SSH flows for each host   &Cross-flow;
 		write/read often\\ 
 		\hline 
 		\hline
 		\multirow{2}{*}{}Portscan detector&Likelihood of being malicious (per host)&Cross-flow; write/read often\\ \cline{2-3} 
 		& Pending conn. initiation req. along with its timestamp & Per-flow; write/read often \\ 
 		\hline 
 		\hline
 		\multirow{3}{*}{}Load& Per server active \# of conn.&Cross-flow; write/read often \\ \cline{2-3} 
 		balancer&  Per server byte counter&Cross-flow; write mostly, read rarely\\ \cline{2-3} 
 		& Conn. to server mapping & Per-flow; write rarely, read mostly \\ 
	\end{tabular}
		\compactcaption{NFs and description of their state objects	}
		\label{ts:nf-state}
\vspace{-0.1in}
\end{table}

{\bf NAT:} maintains the dynamic list of available ports in
the datastore. \JK{When a new connection arrives, it obtains an available
port from the datastore (The datastore pops an entry from the list of available ports on behalf of the NF)}. It then updates: 1) per-connection
port mapping (only once) and, 2)  (every packet) L3/L4 packet counters.

{\bf Portscan detector}~\cite{trw}:  detects
infected port scanner hosts. It tracks new connection
initiation for each host and whether it was successful or not. On each
 connection attempt, it updates the
likelihood of a host being malicious, and blocks a host when the
likelihood crosses a threshold.

% and compares this against statistics from other hosts.  If the We
%implemented this NF using two logical vertices -- firewall and
%analyzer.
%%  One forwarder
%% vertex processes the traffic and keeps track of new connection
%% initiation. For each host, it maintains the 1) likelihood ratio and 2)
%% a queue of connections which have not received a response yet.  An
%% analyzer computes the total likelihood ratio for a host and compares
%% it with the average ratio of all the other hosts. 
%The datastore
%manager notifies the firewall whenever the analyzer updates the
%decision to block a host.

{\bf Trojan detector:} implementation here follows~\cite{lorenzos_work}.


{\bf Load balancer:} maintains the load on each
backend server. Upon a new connection, it
obtains the IP of the least loaded server from the datastore and
increments load. It then updates: 1) connection-to-server mapping
2) per server \#connections and, 3) (every packet) per server byte counter
.

%% , and the
%% mapping between the connection and state object

%%The appendix discusses other \name features.






  


==> paper - Copy/intro.tex <==
\vspace*{-.1in}
\section{Introduction}
\label{sec:intro}

%% Many large networks, including enterprises, telcos, ISPs and data
%% centers, rely on network functions (NFs) to realize sophisticated
%% objectives related to security, compliance, and
%% performance~\cite{}. Whereas NFs were traditionally deployed in
%% custom hardware

NFV vastly improves network management. It allows operators to
implement rich security and access control policies using NF
chains~\cite{nfvwhitepaper,flowtags,boucadair2013differentiated,etsi,nsh}. Operators
can overcome NF failure and performance issues by spinning up
additional instances, and dynamically redistributing
traffic~\cite{gember2013stratos,ftmb}.

To be applicable to enforcing policies correctly, NFV must provide
{\em chain output equivalence} (COE): given an input packet stream, at
any point in time, the collective action taken by all NF instances in
an NFV chain (\figref{fig-physical-chain}) must match that taken by an
hypothetical equivalent chain with infinite capacity always available single NFs (\figref{fig-logical-chain}). COE must hold under dynamics:
under NF instance failures/slowdowns, traffic reallocation for load
balancing/elastic scaling, etc. Given that NFV is targeted for cloud
and ISP deployments, COE should not come at the cost of {\em
performance}.

These goals are made challenging by NFs' {\em statefulness}.  Most NFs
maintain detailed internal state that could be updated as often as per
packet. Some of the state may be shared across instances. For example,
the IDS instances in Figure~\ref{fig-physical-chain} may share {\em
  cross-flow state}, e.g., per port counters. They may also maintain
{\em per-flow} state, e.g., bytes per flow, which is confined to
within an instance.


Ensuring COE under statefulness requires that, as traffic is being
processed by many instances, or being reassigned across instances,
updates to state at various NFs must happen in a ``correct''
fashion. For example, shared state updates due to packets arriving at
IDS1 must be reflected at IDS2; likewise, when reallocating a flow,
say $f_1$, from IDS1 to 2, $f_1$'s state should be updated due to
in-flight $f_1$ packets arriving at both IDSes 1 and 2. Finally, {\em
  how} the state is updated can determine an NF's action. For example,
the off-path Trojan detector~\cite{lorenzos_work} in Figure~\ref{fig-example-trojan} relies
on knowing the exact order in which connection attempts were
made. When there is a discrepancy in the order observed w.r.t. the
true order -- e.g., due to intervening NFs running slow or failing --
the Trojan detector can arrive at incorrect decisions, violating COE.




Many NFV frameworks exist
today~\cite{ftmb,pico,splitmerge,E2,OpenBox,statelessnf,S6}. Several of
them focus on managing NF state migration or updates upon traffic
reallocation during scaling or
failover~\cite{ftmb,pico,splitmerge,opennf,S6}. However, they either violate COE, or suffer from poor performance (or both).

%% suffer
%% from key drawbacks that render them unsuitable for modern NFV
%% deployments.
\begin{figure}[t!]
%	\vspace{-1.7em}
	\centering 
	\subfloat[][]{%
		\label{fig-physical-chain}	
		\includegraphics[scale=0.65]{figures/physical_chain.pdf}%
	}
	\subfloat[][]{%
		\label{fig-example-topo}
		\label{fig-logical-chain}		
		\includegraphics[scale=0.65]{figures/logical_chain.pdf}%
		
	}
	
	
	
	\compactcaption{(a) Example NFV chain with many instances per NF (b) logical view with infinite capacity NFs/links for COE.}
	\label{fig-nfv-chain}
	\vspace{0.3em}
\end{figure}
%% , and focus exclusively on
%% state confined entirely within an instance.
First, most systems {\bf ignore shared
  state}~\cite{ftmb,pico,splitmerge,E2}.  They assume
that NFs do not use cross-flow state, or that traffic can be split
across NF instances such that sharing is completely
avoided. Unfortunately, neither assumption is valid; many
NFs~\cite{broids,squid,re,prads} have cross-flow state, and the need
for fine-grained traffic partitioning for load balancing can easily
force cross-flow state sharing across instances. Because shared state is
critical to NF processing, ignoring how it is updated can lead to
inconsistent NF actions under dynamics, violating COE (\secref{today}).


Second, existing approaches {\bf cannot support chain-level
  consistency}. They cannot ensure that the order of updates made to
  an NF's state (e.g., at the Trojan detector~\cite{lorenzos_work}
  in~\figref{fig-example-trojan}) are consistent with the input packet
  stream. This inability can lead to NFs arriving at incorrect
  decisions, e.g., missing out on detecting attacks (as is the case
  in~\figref{fig-example-trojan}), violating COE. Similar issues arise
  in the inability to correctly suppress spurious duplicate updates
  observed at an NF due to recovery actions at upstream NFs
  (\secref{requirements}).
  %% or triggering
%% false alarms due to spurious duplicates that arise during failure
%% recovery. \aditya{duplicate suppression is not clear}

%The above two drawbacks mean that existing frameworks cannot support COE.

Finally, existing frameworks impose {\bf high overhead} on state
maintenance, e.g., 100s of milliseconds to move per-flow state 
across instances when traffic is reallocated (\secref{today}).

We present a new NFV framework, \name (``correct, high-performance
chains''), which overcomes these drawbacks. For COE, \name uses three
building blocks. \name stores NF state in an in-memory
{\bf external state store}. This ensures that state continues to be
available after NF instances' recover from failure, which is necessary
for COE. Second, it maintains simple {\bf metadata}. It adds a
``root'' at the entry of a chain that: (1) applies a unique logical
clock to every packet, and (2) logs packets whose processing is still
ongoing in the chain. At the store and NFs, \name tracks packet clocks
along with update operations each NF issues. Clocks help NFs to reason
about relative packet ordering irrespective of intervening NFs'
actions, and, together with datastore logs, help suppress
duplicates. We develop failure recovery protocols which leverage
clocks and logs to ensure correct recovery from the failure. In
Appendix \ref{proofs}, we prove their correctness by showing
that the recovered state is same as if no failure has occurred,
thereby ensuring COE. 

State externalization can potentially slow down performance of state
reads/writes.  Thus, for performance, \name introduces {\bf NF-aware
algorithms} for shared state management. It uses scope-awareness of
state objects to partition traffic so as to minimize cross-instance
shared state coordination. It leverages awareness of the state access
patterns of NFs to implement strategies for shared state
caching. Because most NFs today perform a simple set of state update
operations, \name offloads operations to the state store, which
commits them in the background. This speeds up shared state updates
%% (w.r.t. using pairwise coordination~\cite{ftmb,opennf}, or global
%% locks~\cite{statelessnf})
-- all coordination is handled by the store which
serializes the operations issued by multiple NF instances.

%\JK{To ensure COE, 
%Upon NF failure, replaying
%logged packets from the root helps ensure that state updates due to
%packets that were in-flight at the time of failure are also
%handled. Finally, we show that clocks and NF-side logs help ensure COE
%even under datastore failure/recovery.

We built a multi-threaded C++ prototype of \name along with
four NFs. We evaluate this prototype using two campus-to-EC2
packet traces.  \JK{We find that \name's state management optimizations
reduce latency overhead to {\bf 0.02$\mu$s - 0.54$\mu$s} per packet
compared to traditional NFs (no state externalization).} \name failover offers {\bf 6X} better
75\%-ile per packet latency than~\cite{ftmb}. \name is 99\% faster in
updating strongly consistent shared state, compared to
~\cite{opennf}. \name obtains per-instance
throughput of 9.42Gbps -- {\bf same as maximum achievable} with
standalone NFs. \name's support for chain-wide guarantees adds little
overhead, but {\bf eliminates false positives/negatives} seen when
using certain security NFs in existing NFV frameworks. Thus, \name is
the only framework to support COE, and it does so at state-of-the-art
performance.

%% \aditya{implementation details on storm}

%% \aditya{results summary}


==> paper - Copy/motivation-nsdi.tex <==
\section{Motivation}

\label{s:mot}

NFV allows operators to connect NFs together in chains, where each
type of NF can use multiple instances to process input traffic
demand. Use of software NFs and SDN~\cite{simple} means that when
incoming traffic load spikes, or processing is unbalanced across 
instances, operators can scale up by adding NF instances and/or
reallocate flow processing  across
instances. Furthermore, hot-standby NFs can be used to continue packet
processing when an instance crashes. Due to these benefits, cloud
providers and ISPs are increasingly considering deploying NFV in their
networks~\cite{etsiwhitepaper}.

%% Since the NFs are typically run in
%% software, they cannot handle arbitrary load -- high
%% volume/pathological traffic can degrade throughput and latency. They
%% are susceptible to crashes, as well as soft failures (e.g., slow downs
%% due to resource contention).  Thus, NFV frameworks need to be able to
%% scale up NFs to handle load, and add backup/recovery instances under
%% failures.

  

\subsection{Key Requirements for COE}
\label{requirements}

NFV chains are central to security and compliance policies,
they must always operate correctly, i.e., ensure COE
(\secref{sec:intro}).  Ensuring COE is challenging: (1) NFs are stateful; they maintain state objects for individual and group of flows. These state objects may be updated on every packet and the value of these state objects may be used to determine the action on the packet. This requires support for fine gained NF state management. (2) In addition to this, COE also require that the per-NF and chain-wide state updates are consistent with the input packet stream.
(3) Since chaining may create a dependency between the action taken in upstream instances and its downstream instances, it is important that the impact of a local action taken for failure recovery should be isolated from the rest of the chain. These challenges naturally map to three classes of requirements for supporting COE:

\vspace{0.05in}
\noindent {\bf State Access:} The processing of each packet requires
access to up-to-date state; thus, the following requirement are 
  necessary to ensure COE under dynamics:

$\bullet$ (R1) {\em State availability:} When an NF instance fails, all state it
has built up internally disappears. For a failover instance to take
over packet processing it needs access to the state that the failed
instance maintained just prior to crashing.

$\bullet$ (R2) {\em Safe cross-instance state transfers:} When traffic is
reallocated across NF instances to rebalance load, the state
corresponding to the reallocated traffic (which exists at the old
instance where traffic was being processed) must be made available at
the reallocated traffic's new location.

\vspace{0.05in}\noindent {\bf Consistency:} Action taken by a given NF
instance may depend on shared-state updates made by other instances of
the same NF, or state actions at upstream NFs in the chain. Ensuring
that said NF instances' actions adhere to COE boils down to following
requirements:

%Ensuring consistency between state updates and input packets boils down to following requirements:

%\begin{compactitemize}

%\item[(R1)] {\em State availability:}



%% Crucially, updates to state due to packets that were in transit to
%% the old instance prior to redistribution must be reflected in the
%% state at the new location~\cite{opennf}.

$\bullet$ (R3) {\em Consistent shared state:} Depending on the nature
of an NF's state, it may not be possible to completely avoid sharing a
subset of it across instances, no matter how traffic is partitioned
(e.g., port counts at the IDSes in~\figref{fig-physical-chain}). Such
state needs to be kept consistent across the instances that are
sharing; that is, writes/updates made locally to shared state by
different instances should be executed at all other instances sharing
the state in the same global order. Otherwise, instances may end up
with different views of shared state leading to inconsistent and hence
incorrect actions.
\begin{figure}[t]
	
	%\vspace{-0.3cm}
	
	\centering
	\includegraphics[width=0.29\textwidth]{figures/trojan-detector.pdf}
	\compactcaption{Illustrating violation of chain-wide ordering.}
	\label{fig-example-trojan}
	
	\vspace{0.2em}
\end{figure}

$\bullet$ (R4) {\em Chain-wide ordering:} Some NFs rely on knowing the order in
which traffic entered the network.
Consider~\figref{fig-example-trojan}. The off-path Trojan
detector~\cite{lorenzos_work} works on a copy of traffic and
identifies a Trojan by looking for this sequence of steps:
(1) open an SSH connection; (2) download HTML, ZIP, and EXE files over
an FTP connection; (3) generate IRC activity. When a Trojan is
detected, the network blocks the relevant external host. A different
order does not necessarily indicate a Trojan. It is crucial that the
Trojan detector be able to reason about the true arrival order as seen
at traffic input.

%% Suppose this NF is preceded by an off-path traffic scrubber NF with
%% two instances; each scrubber reassembles packet payloads and gathers
%% content signatures per flow.
%% and forwards
%% connection information (flow records, and corresponding application
%% headers and content signatures) to the Trojan detector.
In~\figref{fig-example-trojan}, either due to one of the scrubbers
being slowed down due to resource contention or recovering from
failure~\cite{ftmb}, the order of connections seen at the Trojan
detector may differ from that in the traffic arriving at the input
switch.  Thus, the Trojan detector can either incorrectly mark Trojan
traffic as benign, or vice versa.  When multiple
  instances of the Trojan detector are used, the problem is compounded
  because it might not be possible to partition traffic such that all
  three flows are processed at one instance.

%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=0.32\textwidth]{figures/trojan-detector.pdf}
%		\compactcaption{Illustrating violation of chain-wide ordering.}
%		\label{fig-example-trojan}
%	\end{center}        
%	%	\vspace{-1.2em}
%\end{figure}

$\bullet$ (R5) {\em Duplicate suppression:} In order to manage
straggler NFs, NFV frameworks can (a) deploy clones initialized with the
state of a slow NF instance; (b) use packet replay to bring the clone up
to speed with the straggler's state since state initialization; and (c) replicate packets to the straggler and clone (\secref{straggler}). Depending on when the
clone's state was initialized, replay can lead to duplicate state
updates at the straggler. Also, the original and clone instances will
then both generate duplicate output traffic. Unless such duplicate
updates and traffic are suppressed, the actions of the straggler and
of downstream NFs can be impacted (spurious duplicates may trigger an
anomaly). The need for duplicate suppression also arises during fault
recovery (\secref{s:ft-in}).

\vspace{0.05in}
\noindent
{\bf Isolation:} NFs in a chain should not be impacted by failure
recovery of NFs upstream from them. Specifically:

$\bullet$ (R6) {\em Safe chain-wide recovery:} When NF
failures occur and recovery takes place, it is
important that the state at each NF in the
chain subsequent to recovery have the same
value as in the no-failure case. In other
words,  actions taken during
recovery should not impact the processing, state,
or decisions of NFs upstream or downstream
from the recovering NF --- we will exemplify
this shortly when we describe failings of
existing systems in meeting this
requirement.

%% (R6) {\em Cross-NF analysis:} Consider the example
%%               in~\figref{fig-example-crossnf} where the on-path
%%               firewall logs for each host the number of (un)successful
%%               connection attempts to the host; the application gateway
%%               analyzes request/response payloads (e.g., hashes of
%%               temporally popular content) to drive content delivery;
%%               and the off-path analyzer analyzes both connection
%%               patterns (too many failed connections) and content
%%               payloads (sudden spike in the occurrence of certain
%%               payloads) alongside querying a variety of external
%%               databases to identify attacks. It then configures the firewall to
%%               block attack traffic. The analyzer can leverage the
%%               state that is already being maintained by the other two
%%               NFs.

%%        			\begin{figure}[h!]
%%        				\begin{center}
%%        					\includegraphics[width=0.25\textwidth]{figures/cross-nf.pdf}
%%        					\compactcaption{Illustrating cross-NF analysis.
%%                                         }
%%        					\label{fig-example-crossnf}
%%        				\end{center}   
%%        				\vspace{-0.3em}     
%%        			\end{figure}


%\end{compactitemize}

The network today already reorders or drops packets.  Our goal is to
ensure that NF replication, chaining, and traffic reallocation
together do not induce artificial ordering or loss on top of
network-induced issues. This is particularly crucial for many
important off-path NFs (e.g., DPI engines and exfiltration checkers)
which can be thwarted by artificially induced reordering or loss.

\vspace{-.1in}
\subsection{Related work, and Our Contributions}
\label{today}

A variety of NFV frameworks exist
today~\cite{ftmb,opennf,statelessnf,pico,splitmerge,E2,pga,OpenBox,xomb,comb,flowtags,S6}. We
review their drawbacks below.


{\bf Incomplete support for correctness requirements:} Most existing
frameworks focus on handling requirements R1 and/or
R2. Split/Merge~\cite{splitmerge}, OpenNF~\cite{opennf} and S6~\cite{S6} support
cross-instance state transfers (R2).  FTMB~\cite{ftmb} and Pico
Replication~\cite{pico} focus on state availability
(R1).

More fundamentally, Split/Merge, Pico Replication and FTMB focus on
availability of the state contained entirely within an NF
instance. They either ignore state shared across instances, or focus
on the small class of NFs where such state is not used. Thus, these
frameworks cannot handle R3.

\JK{Among existing frameworks, only OpenNF and S6 can support
consistency for shared state (R3), but this comes at high performance
cost. For example, OpenNF imposes a 166$\mu$s per packet 
overhead to ensure strong consistency! (\secref{s:eval}). Similarly, S6 cannot support frequent updates to strongly consistent shared state.} 

Equally crucially, all of the above frameworks focus on a single NF; they cannot handle chains. Thus, none of them support chain-wide
ordering (R4).

\JK{Support for R5 is also missing. StatelessNF~\cite{statelessnf} and S6~\cite{S6} update shared state in an external store or remote NF, respectively,
but they do not support atomic updates to all state objects an instance
can access.} Thus, when a clone is created to mitigate a straggler
off-path NF (as outlined above), the straggler may have
updated other state objects that are not reflected in the clone's initialized state. Upon replay, the straggler can make duplicate state updates (likewise, duplicate
packets can also arise). For the same reason, R6 is also violated:
when an NF fails over, replaying packets to bring the recovery NF up to
speed can result in duplicate processing in downstream NFs. 

{\bf State management performance is poor:} FTMB's periodic
checkpointing significantly inflates NF packet processing latency
(\secref{s:eval}). As mentioned above, OpenNF imposes performance
overhead for shared state. The overhead is high even for
cross-instance transfers of per-flow state: this is because such
transfers require extracting state from an instance and installing it
in another while ensuring that incoming packets are directed to the
state's new location. 
%% Other frameworks not
%% discussed~\cite{OpenBox,xomb,comb,E2,flowtags,statelessnf} also fall
%% short for subsets of the reasons above.

%\JK{Furthermore, as none of the stream processing 
%frameworks~\cite{streamscope,sparkstreaming,heron,storm,structuredstreaming,flink,naiad} is designed for 
%handling cross instance state, thus they don't support {\it R4 -- R6}. Most of them also don't 
%intrinsically support {\it R1 -- R3}, the ones which ensure internal state availability, have poor 
%performance for NFs. StreamScope~\cite{streamscope} can result in significant increase in per packet 
%processing latency as it does periodic checkpointing similar to~\cite{ftmb}.}

%\aditya{this should go elsewhere. perhaps in implementation section?}

%\subsection{Contributions Summary}

{\bf Our contributions:} How do we support requirements R1-R6 while
ensuring good state management performance?  Some NFs or operating
scenarios may just need a subset of R1-R6. However, we seek a {\em
  single framework} that meets all requirements/scenarios because,
with NFV becoming mainstream, we believe we can no longer trade-off
general correctness requirements for performance or functionality
(specific NFs). Thus, we identify {\em basic building blocks} and
study how to synthesize them into one framework. \CR{We have set ourselves the ambitious goal of designing a single generic NFV framework to support all of these requirements, though some NFs may only need support for a subset of these requirements.} Building such a
framework is especially challenging because we must carefully deal
with shared state and NF chaining.

Our system, \name, has three building blocks
  (\figref{fig-overview}): We maintain NF state in a {\bf state store
    external to NFs} (\circled{1}; \secref{s:design}).  NFs access the
  store to read/write relevant state objects. This ensures state
  availability (R1). The store's state object metadata simplifies
  reasoning about state ownership and concurrency control across
  instances (\circled{2}; \secref{storage-sec}). This makes state
  transfer safety (R2) and shared state consistency (R3) simple and
  efficient (\secref{g:scaling}).

%% We insert per packet logical clocks (\circled{2};
%% \secref{runtime-management}). These two basic building blocks help support state
%% availability (R1), and cross-instance ordering (R4).  We embellish
%% these with two additional building blocks, {\em NF-aware state management algorithms} and {\em metadata maintenance} to satisfy the remaining requirements at high performance.}



\begin{figure}[t!]
	\centering 
	\subfloat[][]{%
		\includegraphics[width=0.35\textwidth]{figures/arch.pdf}
%		\compactcaption{Architecture overview.}
		\label{fig-overview}
		\label{fig-dag-mngnt}
	}
	\subfloat[][]{%
		\includegraphics[width=0.07\textwidth]{figures/physical_dag_comp.pdf}%
%
%		\compactcaption{DAGs for the example  in
%			\figref{fig-example-topo}.}
		\label{fig-dag}
		\label{fig-dag-phy} 
		
	}
	
	
		\vspace{-0.3em}
	\compactcaption{(a) \name architecture; (b) Physical chain that \name runs.}
%	\vspace{0.3em}
\end{figure}


%\begin{figure}%[b!]
%	\begin{center}
%		\includegraphics[width=0.46\textwidth]{figures/arch.pdf}
%		\compactcaption{Architecture overview.}
%		\label{fig-overview}
%		\label{fig-dag-mngnt}
%	\end{center}  
%	%    \vspace{-1.2em}      
%\end{figure}
%
%
%\begin{figure}%[b!]
%	\begin{center}
%		\includegraphics[width=0.2\textwidth]{figures/physical_dag_comp.pdf}%
%
%		\compactcaption{DAGs for the example  in
%			\figref{fig-example-topo}.}
%		\label{fig-dag}
%		\label{fig-dag-phy} 
%	\end{center}  
%	%    \vspace{-1.2em}      
%\end{figure}


We propose {\bf NF state-aware algorithms} for good state read/write
performance which is a key concern with state externalization. These
include (\secref{storage-sec}): automatic state scope-aware traffic
partitioning to minimize shared-state coordination (\circled{3});
asynchronous state updates for state that is updated often but read
infrequently; this allows packet processing to progress unimpeded
(\circled{4}); NFs sending update operations, as opposed to updated
state, to the store, which simplifies synchronization and
serialization of shared-state updates (\circled{5}); scope- and access
pattern-aware state caching strategies, which balances caching
benefits against making cache updates immediately visible to other
instances (\circled{6}).

Finally, we maintain a small amount of {\bf metadata -- clocks and
  logs}. We insert per packet logical clocks (\circled{7};
\secref{runtime-management}) which directly supports cross-instance
ordering (R4). We couple clocks with logs to support duplicate
suppression (R5; \secref{straggler}) and COE under failover of NFs and
framework components (R6; \secref{s:ft-in}). We log every packet that
is currently being processed at some NF in the chain (\circled{8}).
Logged packets are replayed across the entire chain during
failover. At the state store, we store logical clocks of packets along
with the state updates they resulted in, which aids duplicate
suppression. At each NF, we store packet clocks along with the update
operations issued and the most recently read state value
(\circled{9}). Together with state store snapshots, these NF-side logs
support COE under datastore recovery.

%% , and help in safe recovery of
%% datastore failures. (3) Finally, we add a per-packet field to track
%% the progress of a packet's processing within a chain. This ensures
%% that packets are always processed exactly once even under failures
%% amidst non-blocking updates.

%% \aditya{all of the below needs to be rewritten}

%% \JK{ \name is a
%%   novel NFV framework that satisfies the aforementioned requirements
%%   and challenges. In this section we outline the key ideas and
%%   contributions. In \secref{sec:api}, \secref{s:design} and
%%   \secref{design}, we provide the details.

%% \name provides a high level API (\secref{sec:api}) to network operators to implement NF chains without worrying about the underlying complex details of ensuring fault tolerance, providing straggler mitigation and offering elastic scaling (\secref{g:scaling}, \secref{straggler} \& \secref{faulttolerance}). It leverages scopeawareness to implement novel caching strategies to minimize the cross flow state coordination and to  improve performance and partition traffic (\secref{scope-aware}). It also externalizes the state to provide flexible high performance state management. It uses novel NF specific caching strategies to improve performance. Furthermore, it leverages NF specific state access patterns to offer various state update mechanisms to further optimize the state management (\secref{storage-sec}). It also provides capability to reason about chain wide temporal ordering across flows (\secref{chainwide-ordering}) and a callback based novel approach to support actions which need cross chain state access (\secref{storage-sec}).

%% It also implements a novel state locking mechanism by encoding IDs in the key of state objects to ensure safe handover of per-flow state during elastic scaling (\secref{g:scaling}). It also guarantees state consistency during failure recovery and straggler mitigation process by suppressing duplicate state updates and outputs. Moreover, during this process, it also avoids duplicate processing at upstream NFs in the chain (\secref{straggler} $\&$ \secref{faulttolerance}).

%% }

Though StatelessNF~\cite{statelessnf} first advocated for externalizing
state, but it has serious issues. Aside from a lack of support for
R4--R6, it lacks atomic state updates: when a single NF fails after
updating some but not all state objects, a failover NF can boot up
with incorrect state!  It requires locks for shared state updates,
which degrades performance. Also, it assumes Infiniband networks for performance.

%% \aditya{not sure where to put the following:}

%% Furthermore, as none of the stream processing
%%   frameworks~\cite{streamscope,sparkstreaming,heron,storm,structuredstreaming,flink,naiad}
%%   is designed for handling cross instance state, thus they don't
%%   support {\it R4 -- R6}. Most of them also don't intrinsically
%%   support {\it R1 -- R3}, the ones which ensure internal state
%%   availability, have poor performance for
%%   NFs. StreamScope~\cite{streamscope} can result in significant
%%   increase in per packet processing latency as it performs periodic
%%   checkpointing to ensure fault tolerance.




==> paper - Copy/otherrelatedwork.tex <==
\section{StatelessNF and Some other Works}

\aditya{talk about statelessNF in detail here. and then about other papers.} \junaid{updated}
\JK{  
We note that StatelessNF~\cite{statelessnf} which first 
advocates for externalizing state claims to support R1 as well. However,unfortunately it does not ensure atomic state update nor does it have
have a state rollback mechanism. This can lead to an inconsistent state when an NF fails after updating some of the state
objects. Moreover, it does not provide support for updating shared states. To support consistent updates to shared states, it
requires locks, which can significantly degrades the performance. Unlike \name, low latency networks (RDMA or Infiniband) are crucial for the performance of StatelessNF.



==> paper - Copy/package.tex <==
%\usepackage{oneinchmargins,doublespace,times}
\usepackage{oneinchmargins}
\usepackage{times}
\usepackage{graphicx}
\usepackage{url}
%\usepackage{color}
\usepackage{float}
\usepackage{verbatim}
\usepackage{authblk}
\usepackage{calc}
\usepackage{soul}

%\usepackage[]{hyperref}
%\usepackage[bookmarks=false,breaklinks]{hyperref}
%\usepackage[hyphenbreaks]{breakurl}


\usepackage{setspace}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{wrapfig}
\usepackage{alltt}
\usepackage{epstopdf}
%\usepackage{subfigure}
%\usepackage{pifont}

% for tables
\usepackage{booktabs}
\usepackage{threeparttable}


%\usepackage{bbding}
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
%\usepackage{mathtools}
%\usepackage{listings}
\usepackage{algorithm}
\usepackage{algorithmic}
%\usepackage[noend]{algpseudocode}

\usepackage{tabularx}

\usepackage{fancyvrb}
\usepackage[normalem]{ulem} % for strike out,  \em and \sout are now strikes, use \it for italic
\renewcommand{\ttdefault}{cmtt}

%\usepackage{colortbl} % for table color
\usepackage{pstricks} % for gray hline
%\input{colortab} % for gray hline (must include pstricks)
\usepackage{array}

\usepackage{textcomp}

\usepackage{enumerate}
\usepackage[shortlabels]{enumitem}
\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

\usepackage[normalem]{ulem}  % for strike through



==> paper - Copy/runtime.tex <==
\section{Correctness}
\label{design}
\label{runtime-management}

So far, we focused on state management and its performance. We also
showed how \name supports requirement R1 (state availability) by
design.  We now show how it supports the requirements R2--R6. This is
made challenging both by shared state and by chaining. To support
R2-R6, \name maintains/adds metadata at the datastore, NFs and to
packets. We first describe how the most basic of the metadata --
logical packet clocks and packet logs -- are maintained. We describe
other metadata along with the requirements they most pertain to.

%% \name's framework manager supports fault tolerance
%% (e.g., automatically spin up backup NF instances), as well elastic
%% scaling and straggler mitigation (automatically deploy/decommission NF
%% instances based on vertex manager guidance). In doing so, it uses the
%% above building blocks to perform necessary underlying state
%% management. However, it needs two additional mechanisms to ensure
%% chain equivalance in such dynamic situations---

%% to ensure chain
%% equivalance in the face of dynamics such as traffic reallocation,
%% traffic duplication or failure.

%% \name's framework manager supports high performance NF
%% chains while preserving chain equivalence. It
%% leverages the building blocks (Section~\ref{s:design}) to: (a)
%% react to hard failures by bringing up new instances, (b) react
%% to soft failures by killing or duplicating  stragglers,
%% and (c) scale up (add) instances to meet demand and scale down
%% for cost-efficiency.

%% Two key mechanisms -- creation/use of logical clocks, and packet
%% logging -- aid the framework manager in ensuring chain equivalence.
%when performing the above activities.%%  We describe them below, and then
%% address how they are used.

%% , as well as managing the lifecycle of physical DAG's NF
%% instances.

%% Specifically, it ensures elastic scaling (by adding/remove
%% NF instances), fault tolerance (by replaying traffic upon failures of
%% instances) and straggler mitigation (by replicating or
%% killing/restarting slow NF instances) for the physical DAG.
%% Users can customize the logic used for each of these three aspects by
%% providing modules for each of them.  These modules work on the global
%% view of the DAG by taking the hints from all the {\em vertex managers}
%% as input. The vertex manager, shown in \figref{fig-dag-mngnt},
%% inspired by Tez~\cite{tez}, is responsible for collecting statistics
%% from each vertex to provide hints to the framework (e.g., for scale
%% up/down or straggler mitigation). These hints are customizable
%% through user defined modules. The user can also provide custom
%% implementation of the hints generator.

%% In response to the output of these modules, the framework manager
%% deploys additional instances/terminates existing ones as needed, and
%% updates the communication patterns/routes to re-distribute the traffic
%% along with the state handover/transfer (discussed in section
%% \ref{design}).

%% In this section, we describe how our framework handles runtime issues
%% related to fault tolerance, accuracy and performance. These issues
%% include state management during scaling, handling state updates and
%% duplicate output during straggler mitigation, reprocessing of input
%% after a failure, and ensuring ordering across different
%% instances.

{\bf Logical clocks, logging:} The root (\secref{scope-aware})
attaches with every input packet a unique {\em logical clock} that is
incremented per packet.  The root also {\em logs} in the datastore
each packet, the packet clock, and to which immediate downstream
instance the packet was forwarded.  When the last NF in a chain is
done processing a packet, updating state and generating relevant
output, it informs the \name framework. \name sends a ``delete''
request with the packet's clock to the root which then removes the
packet from the log. Thus, at any time, the root logs all packets that
are being processed by one or more chain instances. \JK{When any NF in the
chain cannot handle the traffic rate, the root log builds in size; CHC
drops packets at the root when this size crosses a threshold to avoid
buffer bloat.} When multiple root instances are in use
(\secref{scope-aware}), we encode the identifier of the root instance
into the higher order bits of the logical clock inserted by it to help
the framework deliver ``delete'' requests to the appropriate root
instance.


% We
%assume that NFs that are not connection-terminating don't modify the
%logical clock passed with a packet.\footnote{NF authors can ensure
%  this.} The splitter immediately downstream from a connection
%terminating NF also acts as a root splitter: adds it own logical clock
%and logs the packets it outputs.

%The logical clock added by the splitter at the root vertex is
%``consumed'' at the most immediate downstream {\em connection
%  terminating} NF (acting as a TCP endpoint, e.g., an application
%gateway): such an NF informs the \name framework that it is done
%processing a packet, updating state and generating relevant
%output. The framework sends a ``delete'' request with the packet's
%logical clock to the upstream root splitter; then the packet is removed
%from the log. Thus, the root splitter stores all packets (locally or
%at the datastore) that are being processed by one or more instances
%between itself and a downstream connection terminating instance.  We
%assume that NFs that are not connection-terminating don't modify the
%logical clock passed with a packet.\footnote{NF authors can ensure
%  this.} The splitter immediately downstream from a connection
%terminating NF also acts as a root splitter: adds it own logical clock
%and logs the packets it outputs.

 %% Alternately, or as a fail-safe, the framework can match
 %%  incoming and outgoing packets by computing a Rabin
 %%  Fingerprint~\cite{rabin} over contents~\cite{simple} and ensure
%%  matching packets have the same logical clock.

%% \footnote{To rebalance load across root splitters, a
%%   slice of non-overlapping traffic can be moved from one to another as
%%   long as the new downstream NFs all have access to the required state
%%   from the state store.}


%% In such cases, the
%% Network operators can program their network controllers  to perform scope-aware partitioning across root splitters. The network controller can leverage the { \it .flowspace()} function to determine the scope of each root splitter. \aditya{this is not clear} \JK{is it clear now?}


%% \aditya{This is
%%   incorrect. It seems that queues need to be associated with paths and
%%   not just the downstream tasks} \JK{Last task removes the packet from the datastore. Only packets which belong to the crashed instance, will remain in the datastore ( + in-transit packets). we dont need path information, if partitioning is deterministic } \aditya{this is still not correct. Suppose there are multiple paths to go from root to failed task. How will the root know which path to use. Also this becomes more complex when say two tasks A and B fail.} \JK{In the worst case, we will reply all the traffic till the point of crash. The alternate solution would be to keep track of logical clocks at each splitter. }


%% These all are general distributed system issues. In the
%% rest of this section we describe what are the unique challenges arise
%% in context of packet processing applications and how we overcome them.



\input{scaling}
\subsection{R4: Chain-wide ordering}
\label{add}
\label{trojan_example}
\label{chainwide-ordering}

To support R4, we require that:
{\em Any NF in a chain should be able to process packets, potentially spread
  across flows, in the order in which they entered the NF chain.}
\name's logical clocks naturally allow NFs to reason about
cross-flow chain-wide ordering  and satisfy R4. E.g., the
Trojan detector from \secref{requirements} can use packets' logical clocks to
determine the arrival order of SSH, FTP and IRC connections.
%% ;  consider a more complex
%% situation where multiple instances of the detector are used.
%% %% A naive approach to ensure ordering among flows spread across tasks is
%% %% to synchronize clocks at each worker machine. However, keeping the
%% %% clocks synchronized has a performance overhead. To overcome this
%% %% challenge, we use the logical clock added by the splitter to each
%% %% packet.
%% To reason about ordering across instances, the NF developer can deploy
%% an additional simple analyzer NF that aggregates traffic from the
%% Trojan detector instances and uses packets' logical clocks to
%% determine cross-flow arrival order.

\input{stragglers}
\input{faulttolerance}

%% Typically, when ordering is required, an NF just needs to know the
%% order in which {\em per flow state} is updated across instances, which
%% is supported as above.
%% %% Our logical clocks along with the scope aware partitioning can be
%% %% used to reason about ordering between states of different flows
%% %% processed by different instances, even if the state were cached
%% %% locally.
%% However, our framework cannot ensure ordering
%% between updates to non-perflow state by different instances.


%% Trojan detector in our example can be implemented
%% similar to the IDS in \figref{fig-ids-dag} where forwarders process
%% the traffic and update the per flow information with their logical
%% clock in the datastore. The analyzer reads the state from the
%% datastore, and uses the logical clock values to determine the arrival
%% order of different sessions for its analysis.

%% \aditya{this is incomplete.} \JK{updated}

%% In the appendix, we provide details on \name's support for
%% non-determinstic values, and for synchronous vs. asynchronous NF
%% processing (asynchronous process allows the NF to process a packet
%% without wait for an earlier packet state operation to complete). 



==> paper - Copy/scaling.tex <==
\subsection{R2, R3: Elastic scaling}
\label{g:scaling}

In some situations, we may need to reallocate ongoing processing of
traffic across instances. This arises, e.g., in elastic scaling, where
a flow may be processed at an ``old'' instance and reallocated to a
``new'' scaled up instance.  We must ensure here that the old and new
instances operate on the correct values of per- and cross-flow state
even as traffic is reassigned (requirements R2 and R3). 

Specifically, for cross-flow shared state, we require that: {\em Updates made to the shared state by every incoming packet are
  reflected in a globally consistent order irrespective of which NF
  instance processed the corresponding packet.}

Existing systems achieve this at high overhead: OpenNF~\cite{opennf}
copies shared internal state from/to the instances sharing it, each
time it is updated by an incoming packet! In contrast, ensuring this
property in \name is straightforward due to externalization and
operation offloading (\secref{storage-sec}): when multiple instances
issue update operations for shared state, the datastore serializes
the operations and applies in the background. All subsequent accesses to the
shared state then read a consistent state value.

Per-flow state's handling must be correctly reallocated across
instances, too (R2).  One approach is to disassociate
the old instance from the state object (by having the instance remove
its instance{\_}ID from the object's metadata) and associate the new
instance (by adding its instance{\_}ID).  But, this does not ensure
correct handover when there are in-transit packets that update the
state: even if the upstream splitter immediately updates the
partitioning rules and the traffic starts reaching the new instance,
there might be packets in-transit to, or buffered within, the old
instance. If the new instance starts processing incoming packets right
away then state updates due to in-flight/buffered packets may be disallowed
by the datastore (as a new instance is now associated with the state
object) and hence the updates will be lost.

Thus, to satisfy R2, we require: {\em Loss-freeness, i.e., the state
  update due to every incoming packet must be reflected in the state
  object.} Furthermore, some NFs may also need {\em
  order-preservation: updates must happen in the order of packet
arrivals into the network}.

  These properties are crucial for off-path NFs, e.g., IDS. Such NFs
  cannot rely on end-to-end retransmissions to recover from lost
  updates induced by traffic reallocation~\cite{opennf}. Similarly,
  they may have to process packets in the order in which they are
  exchanged across two directions of a flow, and may be thwarted
  by a reordering induced by reallocation (resulting in false
  positives/negatives).

\begin{figure}[t!]
	\begin{center}
		\includegraphics[width=0.45\textwidth]{figures/scaling.pdf}
		\compactcaption{State handover.}
		\label{fig-scaling}
	\end{center}   
	\vspace{-0.2in}     
\end{figure}

\figref{fig-scaling} shows the sequence of steps \name takes for R2:
\circled{1} The splitter marks the ``last'' packet sent to the old
instance to inform the old instance that the flow has been moved. This
mark indicates to the old instance that it should flush any cached
state associated with the particular flow(s) to the datastore and
disassociate its ID from the per flow state, once it has processed the ``last'' packet.  \circled{2} The splitter
also marks the ``first'' packet from the traffic being moved
to the new instance. \circled{3} When the new instance receives the
``first'' packet, it tries to access the per flow state from the
datastore. If the state is still associated with the old
instance{\_}ID, it registers a callback with the datastore to be
notified of metadata updates. \circled{4} The new instance starts
buffering all the packets associated with the flow which is being
moved.  \circled{5} After processing the packet marked as ``last'',
the old instance flushes the cached state and updates the metadata to
disassociate itself from the state. \circled{6} The datastore notifies
the new instance about the state handover.  \circled{7} The new
instance associates its ID with the state, and flushes its buffered
packets.

The above ensure that updates are not lost {\em and} that they
happen in the order in which packets arrived at the
upstream splitter. In contrast, OpenNF provides {\em separate
  algorithms} for loss-freeness and order-preservation; an NF author
has the arduous task of choosing from them!
%% has to choose from, which is not easy as it
%% requires detailed knowledge about the different scenarios in which the
%% designer envisions the NF being used.

Note also that packets may arrive out of order at a {\em downstream}
instance, causing it to make out-of-order state updates. To prevent
this: \circled{8} The framework ensures that packets of the moved flow emitted
by the new instance are not enqueued at the downstream instance, but
instead are buffered internally within the framework until the 
packet marked as ``last'' from the old instance is enqueued at
the new instance.



==> paper - Copy/statemanagement.tex <==

\section{Traffic and State Management}
\label{s:design}

We discuss how \name processes traffic and manages state.  The
framework automatically partitions traffic among NF instances
(\secref{scope-aware}) and manages delivery of packets to downstream NFs (\secref{comm}). As packets flow, different NFs
process them and update state in an external store; \name leverages
several algorithms for fast state I/O; the main challenge here is
dealing with shared state (\secref{storage-sec}).
%\vspace*{-0.5in}
\subsection{Traffic partitioning} 
\label{scope-aware}


%% In what follows, we describe the mechanisms employed by our framework
%% for partitioning/aggregation. \aditya{perhaps communication should go
%%   a different section? implementation?} We then describe how it
%% supports communication among tasks.

%% %% It manages
%% %% partitioning/aggregation of traffic across NF instances, and
%% %% manages communication between them. It also manages the lifecycle of
%% %% vertices; it is responsible for the placement, initialization, scale
%% %% up/down, fault detection and termination of the instances each vertex.

%\subsubsection{Scope-aware partitioning, and Splitters}
\name performs {\em scope-aware partitioning}: traffic from an
upstream instance is partitioned across downstream instances such
that: (1) each flow is processed at a single instance, (2) groups of
flows are allocated to instances such that most state
an instance updates for the allocated flows is not updated by
other instances, and (3) load is balanced. \#1 and \#2 reduce
the need for cross-instance coordination for shared state.


%% \footnote{Other work has
  %% used program analysis tools to infer flowspaces and perform
  %% scope-based partitioning~\cite{statealyr,lorenzos_work}, but our job
%% is easier as the relevant input is available directly.}

%% To support this, \name leverages the flowspace information
%% associated with each state object as follows.
%(lines 6,8; \figref{fig-dag-code})

In \name, state scope is a {\em first-class entity}.  A function { \it
  .scope()} associated with a vertex program returns a list of scopes
i.e., the set of packet header fields which are used to key into the
objects that store the states for an NF; i.e., these are the different
granularities at which states can be queried/updated. \name orders the
list from the most to least fine grained scope. Suppose the DPI vertex
in \figref{fig-example-topo} has two state objects: one corresponding
to records of whether a connection is successful or not; and another
corresponding to the number of connections per host. The scope for the
former is the 5-tuple ({\it src IP, dst IP, src port, dst port,
  protocol}); the scope for the latter is {\it src IP}.

\name first attempts to partition traffic at instances immediately
upstream (which, for the DPI in~\figref{fig-example-topo} would be the
IDSes) based on the most coarse-grained state scope (for the DPI this
is {\it src IP}); such splitting results in no state sharing at the
downstream (DPI) instances. However, being coarse grained, it may
result in uneven load across instances. The framework gathers this
information via the (DPI) vertex manager. It then
considers progressively finer grained scopes and repeats the above
process until load is even. %% In the worst case, traffic is split at the
%% finest scope (e.g., connection 5-tuple).

%% \footnote{Which inevitably means
  %% state pertaining to number of connections per host is shared across
  %% instances.}
  %\aditya{REWROTE THIS. PLEASE CHECK}

%\aaron{which of the
  %scope example you gave is coarser?}

The final scope to partition on is provided in common to the {\em
  splitters} upstream. The framework inserts a splitter after every NF
instance (\figref{fig-dag-phy}). The splitter partitions the output
traffic of the NF instance to instances downstream.
%% \aaron{How do packets modifications made by an NF impacts splitter? How does this relate to SIMPLE ? How does it relate to SFC header from IETF?}

The {\em root} of a physical DAG is a special splitter that receives
and splits input traffic. Roots can use multiple instances to handle
traffic; in \name, we fix root parallelism to some constant $R$.
Network operators are required to statically partition traffic among
the $R$ roots such that the traffic processed by a root instance has
no overlap in any of the 5-tuple dimensions with that processed by
another instance.

%% : it
%%  additionally computes logical packet timestamps and performs packet
%%  logging (\secref{runtime-management}). 

 %% \aditya{this parsed info stuff
 %%   is again never used after this. also, how is the root vertexes
 %%   parsed info passed downstream? how does it help?}\JK{adding metadata to packet. }

 %%  2) It logs all the input packets in the datastore. These
 %% logged packets are used to replay the traffic in case of a failure
 %% (\aditya{refer to a section}).

%% , i.e., {\it src IP address}es.
%% If processing all the traffic on a single not is possible, \aditya{how
%%   would you know this??} it considers progressively finer grained
%% flowspaces. %% and tries to process all the traffic of a particular
%% flow on
%% %% the same instances so that different vertices do not have to share per
%% %% flow state.


%% The function { \it .flowspace()} in line 7 and 9 in \figref{fig-dag-code} returns a list of state objects' flowspace (set of packet header fields) which are used to store the states for the particular NF (vertex). The list is ordered from the most fine grained flowspace to the most coarse grained one. In our IDS example, it returns [{\it (src\_ip,dst\_ip,src\_port,dst\_port,proto),(src\_ip)}].


%% Optionally, a user can provide a custom data partitioner. This takes
%% as input the list of downstream tasks in the physical DAG, and the
%% output flows produced by the given task. It uses the packet header
%% fields in the task's output to determine which downstream task to
%% forward a packet to and configures the splitter accordingly.


%% Note that partitioning applies to both packet and contextual
%% information output by a task.

 %% then produces the IDs of the downstream task in the
%% physical DAG. The framework uses this information to route the output
%% to the appropriate task. \aditya{this seems vague and possibly
%%   incorrect} \JK{downstream tasks gives the possible next hops and task output(packet header) is used for selecting the partition.}

%% } In our example, DPI has a custom user defined partitioning
%%   class(line 8 in \figref{fig-dag-code}).

 \subsection{Communication}
 \label{comm}
 
 Inter-NF communication is asynchronous and non-blocking. Each NF's
 outputs are received by the \name framework which is responsible for
 routing the output to downstream instances via the splitter. The
 framework stores all the outputs received from upstream instances in
 a queue per downstream instance; downstream instances poll the queue
 for input.  This approach offers three benefits: (a) upstream
 instances can produce output independent of the consumption rate of
 downstream instances, (b) the framework can operate on queue contents
 (e.g., delete messages before they are processed downstream), which
 is useful for certain correctness properties, e.g., duplicate
 suppression (\secref{runtime-management}), (c) user logic can use
 persistent queues to identify stragglers/uneven load.
 
%% \aditya{i am talking about a case where an NF
%%    is dependent on two different upstream NFs. Does the downstream NF
%%    have to coordinate on reading/acting on the outputs from the two
%%    upstreams. Also, it would be good to have a richer example upfront
%%    that has such a complex DAG structure.}


%% When multiple users are running their DAGs, the framework manager ensures that each user gets its allocated share of CPU, memory and network resources for each individual task.

\input{storage}
%\input{storage}



%\subsection{Parser}
%To avoid the re-parsing of the packet header for the same information or reconstruction of the same session information multiple times at different stages, the framework adds parser instances. Worker instances register with the parser for their required input events (e.g. IP header, TCP segment, TCP connection setup), the parser parses and collects the required data, and generates events. It might be possible that a worker instance takes both the event from parser, and the output from the upstream worker as an input, in such cases the framework caches the input received by the parser and waits for the output of upstream worker instance. The logical clock associated with the packet header is used as a key to cache the packet in a hash table. The output of upstream worker also contains the corresponding logical clock value which makes it easy to correlate the output of the upstream worker with the cached input. Parser is required to maintain the state for generating high level complex events, in section \ref{avoid-reparsing}, we discussed how this state is recovered in case of a failure.

%% \subsection{Worker}
%% A worker analyzes and potentially modifies the packet. The worker consumes the packet or the output produced by other worker instances as input and updates the state. In \figref{fig-ids-dag}, {\it forwarder} is an example of such a worker. The worker can also consume events generated by the datastore manager. For example, timer or state object update events, such events are usually use for triggering cross flow analysis. The datastore manager notifies the {\it analyzer} whenever the state is updated by the {\it forwarder}.


==> paper - Copy/storage.tex <==
\subsection{State  Maintenance}
\label{storage-sec}

%% Today, NF instances maintain critical state internally.
%% State sharing and coordination are not well supported, leading to poor 
%% performance and lack of fault tolerance.
%% this state can correspond to individual flows (as
%% defined by, e.g., a connection 4-tuple; for instance, a per connection
%% byte counter), or can be shared across groups of input traffic flows
%% (e.g., per port byte counters). As prior systems have recognized,
%% ensures that this state is kept consistent and up-to-date as traffic
%% is reallocated across instances (e.g., during elastic scaling) is
%% challenging and requires heavy-handed mechanisms.

%% \JK{added about stateless NF. Should we move it to related work ?}
%% \aditya{MOVE THIS: similar to Stateless NF~\cite{statelessnf}. Stateless NF assumes that most of the state is read-heavy which is only true for simple NFs (e.g. NAT). It also performs poorly for shared state because of the state access contention between different NF instances. We overcome these issues and generalized the state externalization by offloading state update to datastore}


\name{} {\em externalizes} NF state and stores it in an external
distributed key-value datastore. Thus, state survives NF crashes,
improving availability and satisfying requirement R1
(\secref{s:mot}). All state operations are managed by the datastore
(\figref{fig-overview}). As described below, \name incorporates
 novel algorithms and metadata to improve performance (\tabref{ts:iostrategies}).

%% \JK{Different from~\cite{statelessnf}, we
%%   support operation offloading, non-blocking updates, and various
%%   state caching strategies to further improve performance, and
%%   callbacks; to support actions that need cross-chain state access. In
%%   addition to this, unlike ~\cite{statelessnf}, low latency networks
%%   (Infiniband or RDMA) are not crucial for the performance of
%%   \name}. Before discussing these, we present the metadata maintained
%% with state objects.
\label{metadata}

%% Each NF can use custom organizations of its state objects; however, we
%% expect most state objects to be accessed based on values of packet
%% header fields (which is common practice today).

%% In what follows, we describe the design and key attributes of our
%% state datastore. Later, in Section XXX, we outline how our approach
%% simplifies ensuring state consistency in dynamic
%% reallocation. \aditya{this may need to be rephrased}

%% Our framework externalizes all internal NF state. 

%% To support elastic scaling and high availability, we externalized the internal state of a NF (worker). The storage consists of three parts: a datastore, a datastore manager and a task side library.

%% {\bf Datastore structure and contents:} All state is stored in our
%% datastore. 

%% In addition, every input packet is logged into the data store for a certain period of time.

%% The datastore is an in-memory key value store which stores the internal state and logs the input packets. We leverage common network function access patterns to 
%% store the state. Network functions organize their state in simple data structures (e.g. hash tables or linked lists) and use packet header fields to access the state. %We store the internal state in an in-memory key-value store. We also use key-value store to log the input packet, but key-value store is not necessary for logging packets.  TODO


% \aditya{check this reference to SQL}

\begin{table}[]
	\centering
	%	\setlength{\tabcolsep}{0.5em}
	\scriptsize
	\begin{tabular}{p{0.7cm}||p{1.4cm}|p{1.40cm}|p{1.3cm}|p{1.9cm}}
		Scope& Any&Per-flow&Cross-flow&Cross-flow\\
		
		\hline
		
		Access pattern&Write mostly, read rarely&Any&Write rarely (read heavy)&Write/read often\\
		
		\hline
		\hline
		
		&Non-blocking ops. No caching&Caching \textbackslash w periodic non- blocking flush&Caching \textbackslash w callbacks&Depends upon traffic split. Cache, if split allows; flush periodically \\
	\end{tabular}
	\caption{Strategies for state management performance}
	%\end{scriptsize}
	\vspace{-0.2in}
	\label{ts:iostrategies}	
\end{table}


{\bf State metadata:} The datastore's client-side library appends
metadata to the key of the state that an NF instance stores.  This
contains vertex{\_}ID and instance{\_}ID, which are immutable and are
assigned by the framework. In \name, the key for a per-flow (5 tuple)
state object is: {\it vertex{\_}ID + instance{\_}ID + obj{\_}key},
where obj{\_}key is a unique ID for the state object. The
instance{\_}ID ensures that only the instance to which the flow is
assigned can update the corresponding state object. Thus, this
metadata simplifies reasoning about ownership and concurrency
control. Likewise, the key for shared objects, e.g., {\it
  pkt{\_}count}, is: {\it vertex{\_}ID + obj{\_}key}. All the instances
of a logical vertex can update such objects. When two logical vertices
use the same key to store their state, vertex{\_}ID prevents any
conflicts.



  %% It's design is based on two key insights.
  %% First,


  {\bf Offloading operations:} Most NFs today perform simple
  operations on state. \tabref{t:operations} shows common examples. In
  \name, an instance can {\em offload operations} and instruct the
  datastore to perform them on state on its behalf \JK{(developed contemporarily with ~\cite{S6})}. Developers can
  also load custom operations. The benefit of this approach is that NF
  instances do not have to contend for shared state. The datastore
  serializes operations issued by different instances for the same
  shared state object and applies them in the background (\secref{secproof:crossflow} proves that updates will always result in  consistent state.). This offers
  vastly better performance than the natural approach of acquiring a
  lock on state, reading it, updating, writing it back, and
  releasing the lock (\secref{s:eval}).
\input{tables/operations}
%(we omit syntax for brevity).

%% using following commands:\\
%% \begin{scriptsize}
%% {\em cmd ($<$key$>$,$<$operation\_ID$>$,$<$operation\_args$>$,$<$blocking/non-blocking$>$)}
%% {\em Async\_cmd ($<$key$>$,$<$operation\_ID$>$,$<$operation\_args$>$,$<$callback$>$)} 


%% \end{scriptsize}





%\begin{figure}[t]
%	\vspace{0.3em}
%	\centering \subfloat[][]{%
%		\label{fig-state-update-nv}%
%		\includegraphics[scale=0.5]{figures/state_update_nv.pdf}%
%	}
%	\hspace{0.75em}%\hfill
%	\subfloat[][]{%
%		\label{fig-state-update-offload} 
%		\includegraphics[scale=0.5]{figures/state_update_offload.pdf}%
%	}
%	\vspace{-0.3em}
%	\compactcaption{State updates: (a) locking, (b) \name}
%	\label{fig-}
%\end{figure}
%




\label{IDS-example}

 %% These custom operations are
%% configured during DAG initialization and are assigned an ID. Tasks use
%% these IDs when communicating with the store.


%% Our second insight is that
%% state updates occur in two different types
%% of situations, the more common of which can be optimized given our
%% design. In
\label{g:rexmit}

{\bf Non-blocking updates:} In many cases, upon receiving a packet, an
NF updates state, but does not use (read) the updated value; e.g.,
typical packet counters (e.g.,~\cite{broids,prads,squid}) are updated
every input packet, but the updated value is only read infrequently.
For such state that is written mostly and read rarely, we offer {\em
  non-blocking updates} (\tabref{ts:iostrategies}): the datastore
immediately sends the requesting instance an ACK for the operation,
and applies the update in the background.  As a further optimization,
NFs do not even wait for the ACK of a non-blocking operation; the
framework handles operation retransmission if an ACK is not received
before a timeout. \JK{If an instance wishes to read a value, the
  datastore applies all previous outstanding updates to the value, in
  the order NFs issued them, before serving the read.}

% \aditya{I simplified this
%  description. Make sure it is correct.}


%The datastore manager manages the meta-data and performs the state update operations on the datastore. One of the key benefits of offloading the state update operation is to avoid contention in updating the state. 

%The datastore manager is responsible for serializing the operations received from different task instances for the same state. The datastore manager is an elastically scalable. A single datastore manager instance can be responsible for one or more state objects. 

%% Another insight which we leverage is that NF, either just reads and updates the state object and does not use the updated value or just uses the updated value 
%% of the state object. An example of the former is a packet counter, which each task updates on each input packet, but the task reads the updated value 
%% infrequently after a particular number of packets. To facilitate such cases where the task does not read the updated value, we define non-blocking 
%% operations. The datastore manager sends an ack for such functions after receiving the function and applies them later in the background. An example of the later 
%% type of update is a blocking operation, where the task requires the updated value to further process the packet.


%% As every task has a
%% unique task{\_}ID. The per flow state is only updated by the task to
%% which the flow is assigned for processing, and the per flow state key
%% computed above ensures this property. 
%% The task{\_}ID is used by the
%% datastore
%% manager to associate the state with the task that can update it. It
%% also acts as a lock by preventing other tasks from over writing the
%% state.

\noindent

{\bf Caching:} For all the objects which are not amenable to
non-blocking updates, we improve state access performance using novel
caching strategies that leverage state objects' scope and access
patterns (ready-heavy vs. not).
%and nature (critical vs. not) of state objects,
\label{caching}

{\em Per-flow state:} \name's scope-aware partitioning ensures that flows that update 
per-flow state objects are processed by a single instance; thus, these objects do not have 
cross-instance consistency requirements. The datastore's client-side library caches them at the relevant 
instance, which improves state update latency and throughput. However, for fault tolerance, we require 
local updates made to cached objects to be flushed to the store; to improve performance, these 
flush operations have non-blocking semantics (\tabref{ts:iostrategies}). 
%As a further optimization, we flush 
%cached state as soon as it is updated only if the state is critical (e.g., ``unexpected RST seen for flow 
%$f$''); we flush non-critical local state (state which just impacts the log output e.g., packet counters) infrequently, or once every $N$ 
%updates.\footnote{We expect the developer to identify whether state is critical or not in the config} \junaid{Flushing the cached state periodically decreases the traffic between the store and the NF, but it comes at the cost of increasing the memory required for logging packets for ensuring fault tolerance (\secref{faulttolerance}).}

%% \footnote{To elaborate: our framework
  %% determines the scope aware partitioning at the splitter upstream
  %% from a set of NF instances. Based on this it knows the flowspace of
  %% a downstream task, say $fs$. All state objects whose flowspace is
  %% $fs$ or finer can be safely cached.}

{\em Cross-flow state:} Cross-flow state objects can be updated by
multiple instances simultaneously. Unlike prior works that
largely ignore such state, \name supports high performance shared
state management.  \CR{Some shared objects are rarely updated;
  developers can identify such objects as read-heavy. \name (1) caches such an object at the instances needing them; and (2) the client-side library at each of these instances registers a {\em callback} with the store, which is invoked whenever the store updates the object on behalf of another instance. The NF developer does not need to handle callback to update state; they are handled by the client-side library.}
  
 The cached objects only {\em serve read requests}. Whenever an (rare) update is issued by an instance - operation is immediately sent to the store, The store applies the operation and sends back the updated object to the update initiator. At the same time, the client-side library of other instances receives callback from the store and updates the locally cached value (\tabref{ts:iostrategies}). We prove this approach results in consistent updates to shared state in
 \secref{secproof:cachedcrossflow}.
 
 
% 
%  These objects are
%  cached at instances needing them. These cached objects {\em only
%    serve read requests}. Whenever an (rare) update is issued, the
%  operation is immediately sent to the store to avoid race conditions. The store applies the operation on the state and sends back the updated object.

%Also, for such objects, the client-side library at an instance
%registers a {\em callback} with the datastore, which is invoked
%whenever the store updates the object on behalf of another
%instance. Upon receiving the callback, the client-side library updates
%the cached value (\tabref{ts:iostrategies}).







For other cross-flow objects (not rarely-updated), the datastore
allows them to be cached at an instance only as long as no other
instance is accessing them (\tabref{ts:iostrategies}); otherwise, the objects
are flushed. \name{} notifies the client-side library when to
cache or flush the state based on (changes to) the traffic
partitioning at the immediate upstream splitter.
%	 a flow can be cached and whe,When an access occurs, the
%datastore notifies the client-side library to stop caching that object
%and flush any cached state.

For {\bf scale and fault tolerance} we use multiple datastore
instances, each handling state for a subset of NF instances. \JK{Each datastore instance is multi-threaded. A thread can handle multiple state objects; however, each state object is only handled by a single thread to avoid locking overhead. }

%% ; in fact the library only needs to flush the corresponding state
%% {\em operations}, which imposes far less overhead than flushing {\em
%%   state}.

%% \aditya{cut or move this to footnote: To enable caching of eventually
%%   consistent cross flow state, we recommend developers to split and
%%   store the cross flow state as task level state, {\it if
%%     possible}. For example in case of PRADS~\cite{prads}, a monitoring
%%   NF, instead of keeping track of services running on a host as a
%%   shared cross flow state, each task can keep a task local state and a
%%   separate worker can later aggregate the state for logging.}



%% \begin{figure}[thb!]
%%     \begin{center}
%%     \includegraphics[width=0.4\textwidth]{figures/ids_dag.pdf}
%%     \compactcaption{Cross-NF analysis.}
%%     \label{fig-ids-dag}
%%     \end{center}       
     
%% \end{figure}

%% {\bf Callbacks:} Vertices can register callbacks with the datastore
%% manager for timer and state update events.  The latter can be used by
%% an instance to know about updates to cached cross-flow state (as
%% exemplified above).

%% or for cross-NF coordination (R6;
%% \secref{s:mot}) which we discuss next. Consider the scenario in \figref{fig-example-crossnf}
%% for example. \name supports it as shown in \figref{fig-ids-dag}.
%% %% ; callbacks
%% %% provide simple support for cross-NF coordination needed in this case
%% %% (\figref{fig-ids-dag}):
%% The firewall and gateway, respectively, update per-host (number of
%% (un)successful connections for the host) and per content-hash (whether
%% the frequency count for a content crossed a threshold) state at the
%% store; the analyzer has simple per-host state (on whether to block a
%% host or not). The analyzer registers callbacks (\figref{fig-ids-dag})
%% with the datastore manager to be notified whenever any host's or
%% content hash's state value is updated. Likewise, the firewall
%% registers a callback with the datastore manager to be notified
%% whenever the analyzer updates the decision for a host to be blocked or
%% not. The needed coordination between the analyzer and the
%% firewall/gateway happens indirectly via the datastore. Such
%% coordination is impossible today because NFs can't access each other's
%% state.

 %%We discuss further in~\secref{eval}.


%% On every
%% packet the firewall updates simple per-flow state at the store,
%% depending on whether the host is blocked or not, forwards the
%% packet. The decision of whether to allow or block a particular host is
%% made by the {\it analyzer}. The {\it analyzer} updates the decision in
%% the datastore. The {\it forwarder} registers a callback with datastore
%% manager, which is called whenever the {\it analyzer} updates the
%% decision. The {\it forwarder} does not have to read the decision on
%% every packet from the datastore manager. The datastore manager
%% notifies the {\it forwarder} when the state is updated by the {\it
%%   analyzer}. Similarly the {\it analyzer} just runs whenever the
%% connection attempt count is updated by the {\it forwarder}. 

%%  For the latter, tasks register for updates
%% to specific state objects, and the datastore manager generates events
%% when the state object is modified.

%% \aditya{not sure where to put this example}

%% \aditya{this example does not make sense:

%%   For example, the IPS~\cite{trw} detects port
%% scans and blocks the malicious IP address, if the ratio of
%% unsuccessful to successful connection attempts reaches a threshold. In
%% our framework, such an IPS can be implemented in two parts: a {\it
%%   forwarder}, which processes packets and updates the state, whether
%% the connection attempt was successful or unsuccessful \footnote{The
%%   traffic of a single host can be processed by multiple {\it
%%     forwarders}.}. It does not update any shared state. The second
%% part is the {\it analyzer}. The {\it analyzer} computes the ratio of
%% unsuccessful connection attempts to successful connection attempts for
%% each host. If the ratio is higher than a threshold, it instructs the
%% {\it forwarders} to block that particular host. The {\it forwarder}
%% and the {\it analyzer} does not communicate directly with each other,
%% rather they communicate indirectly through updating state in the
%% datastore.

%% The simplified version of the scan detector is shown in \figref{fig-ids-dag}. The {\it forwarder} process every packet. On every packet {\it forwarder} updates the state and depending upon whether the host is block or not, it forwards the packet. The decision of whether to allow or block a particular host is made by the {\it analyzer}. The {\it analyzer} updates the decision in the datastore. The {\it forwarder} registers a callback with datastore manager, which is called whenever the {\it analyzer} updates the decision. The {\it forwarder} does not have to read the decision on every packet from the datastore manager. The datastore manager notifies the {\it forwarder} when the state is updated by the {\it analyzer}. Similarly the {\it analyzer} just runs whenever the connection attempt count is updated by the {\it forwarder}. The {\it analyzer} register a callback with the datastore manager, the datastore manager notify the {\it analyzer} whenever the value is updated.

%% }





==> paper - Copy/stragglers.tex <==
\subsection{R5: Straggler mitigation}
\label{straggler}
\label{stragglers}
R5 calls for the following:
{\em All duplicate outputs, duplicate state updates, and duplicate
  processing are suppressed.}

A key scenario in which duplicate suppression is needed is straggler
mitigation.  A straggler is a slow NF that causes the entire NF
chain's performance to suffer. We first describe \name's mechanism for
straggler mitigation (which kicks in once user-provided logic
identifies stragglers;~\secref{sec:api}), followed by duplicate
suppression.

{\bf Clone and replay:} To mitigate stragglers \name deploys {\em
  clones}. A clone instance processes the same input as the original
in parallel. \name retains the faster instance, killing the
other. \name{} initializes the clone with the straggler's latest
state from the datastore. It then replicates incoming traffic from the
upstream splitter to the straggler and the clone.

This in itself is not enough, because we need to satisfy R2, i.e.,
ensure that the state updates due to packets that were in-transit to
the straggler at the time the clone's state was initialized are
reflected in the state that the clone accesses. To address this, we
{\em replay} all logged packets from the root. The root continues to
forward  new incoming packets alongside replayed ones. The clone
processes replayed traffic first, and the framework buffers replicated
traffic. To indicate end of replay traffic, the root marks the
``last'' replayed packet (this is the most recent logged packet at the
time the root started replaying).  When replay ends (i.e., the packet
marked ``last'' was processed by the clone), the framework hands buffered
packets to the clone for processing.

Given the above approach for straggler mitigation, there are three
forms of duplicates that can arise. \name suppresses them by
maintaining suitable metadata.

{\bf 1. Duplicate outputs:} Replicating input to the clone results in
duplicate outputs. Here, the framework suppresses duplicate
outputs associated with the same logical clock at message queue(s)
of immediate downstream instance(s).

\begin{figure}[]
	\centering
	\subfloat[][Naive reprocessing]{%
		\label{fig-ft-nv-reproc}%
		\includegraphics[scale=0.57]{figures/ft_nv_reproc_comp.pdf}%
	}
	\hspace{0em}%\hfill
	\subfloat[][Reprocessing with emulation]{%
		\label{fig-ft-reproc} 
		\includegraphics[scale=0.57]{figures/ft_reproc_comp.pdf}%
	}

	\compactcaption{Duplicate update suppression}
%	\vspace{-0.2in} 
	\label{fig-ft}
\end{figure}

{\bf 2. Duplicate state updates:} Some of the replayed packets may have already 
updated some of the stragglers' state objects.  For example, an
IDS updates both the total packet count and
the number of active connections per host. A clone IDS may have been
initialized after the straggler updated the former but not the latter.
In such cases, processing a replayed packet can {\em incorrectly}
update the same state (total packet count) multiple times at the straggler (\figref{fig-ft-nv-reproc}).
To address this, the datastore logs the state value
corresponding to each state update request issued by any instance, as well
as the logical clock of the corresponding packet. This is only done
for packets that are currently being processed by some NF in the chain.
%%\aditya{I CHANGED this: for the reason mentioned
%%  below, I don't think it is enough to keep track of just the last
%%  update}
%% For simplicity of tracking state updates, our framework only allows
%% updating a particular state object once for a given packet.
During replay, when the straggler or clone sends an update for a state object, the
datastore checks if an update corresponding to the logical
clock of the replayed packet has already been applied; if so, the
datastore {\em emulates} the execution of the update by
returning the value corresponding to the update
(\figref{fig-ft-reproc}). \JK{In  Appendix \ref{non-deter}, we describe how \name handles non-deterministic state update operations.}

  %% The manager informs the immediate
  %% upstream root splitter to replay all logged packets whose logical
  %% clock value is greater than the minimum of the logical clock values
  %% of the packets that made the last updates at the failed task's state
  %% objects. }

%% The datastore
%% manager only updates the state if the logical clock value associated
%% with the packet is greater than the logical clock value associated
%% with the last update.
%% It is not possible to get out-of-order updates
%% for a given flow, as all the packets of a single flow are processed by
%% the same task in the same order. Updates to cross flow state can
%% arrive out-of-order, however this is already handled by the
%% application through the logical clock.

%% The above also addresses the second issue: all intervening tasks process the replayed packet to ensure
%% appropriate modifications are made to packet header fields and produce
%% relevant contextual information (if any); the datastore allows them to
%% read the state values corresponding to the replayed packet and
%% emulates any updates as before. 

%% \footnote{We assume that the NF
%%   author implements this minimal logic.}

{\bf 3. Duplicate upstream processing:} NFs upstream from the
clone/straggler would have already processed some of the in-transit
packets. In such cases, reprocessing replayed packets leads to
incorrect actions at upstream NFs (e.g., an IDS may raise false
alarms). %%\aditya{elaborate}.
To address this, each replayed packet is marked and it
carries the ID of the clone where it will be processed. Such
packets need special handling: the intervening instances
recognize that they are not suspicious duplicates; if
necessary, the instances read the store for state corresponding
to the replayed packet, make any needed modifications to the
packet's headers, and produce relevant output;
%%  (both
%% of these could be a function of the state at the time the packet was
%% processed);
the instances can issue updates to state, too, but in such
cases the datastore {\em emulates} updates as before.
%% in particular, the datastore allows them to read
%% the state values corresponding to the replayed packet and emulates any
%% updates as before.
The clone's ID is cleared once it processed the packet.
%\JK{Note during the recovery phase the cross-flow state does not require any locking, all the other NF instances can read and update cross-flow state.}


%% Packets
%% whose clocks fall after this state's last update are replayed from the
%% root splitter to the clone; and, the splitter starts replicating
%% incoming traffic to the clone.   \aditya{seems this assumes some info in
%%   FT section}



%%  -- this logic runs in the vertex
%% manager; it can use, e.g., the relative message queue lengths at NF
%% instance
%% \footnote{In our
  %% implementation, if the queue at an instance is persistently long
  %% across several packets, it is deemed a straggler.}

%% Our framework provides support for both killing/restarting or cloning
%% stragglers. The former approach is used when resource availability is
%% plentiful and a restarted instance can be launched at a location with
%% the needed resources. Kill/restart is similar to how we handle instance
%% failures.


%% When resources are scarce, killing/restarting runs the risk of
%% deploying the restarted instance at a heavily contended location,
%% which may further hurt performance. In such cases, 

%% This allows the clone's processing to catch
%% up with the straggler; the clone and the datastore take actions
%% similar to the situation of task failure. When the replay ends
%% \aditya{when does it end?}  the splitter upstream from the
%% clone/straggler starts replicating all input traffic to either task.
%% \JK{added the following to replace this}

%% Whenever a straggler is observed, our framework {\em clones} it and 
%% starts replicating all the input traffic to either task from the 
%% splitter upstream from the clone/straggler. The clone buffers all the 
%% replicated input traffic till it gets the required state. The clone is 
%% instantiated with the straggler's latest state available in the data 
%% store, and all packets whose clocks fall after this state's last 
%% update are replayed to the clone. This allows the clone's processing to 
%% catch up with the straggler; the clone and the datastore take actions 
%% similar to the situation of task failure. The clone starts processing 
%% the buffered traffic after processing the last replayed packet.

 %% an NF may produce output on every packet,

% (\figref{fig-straggler}).
%% downstream task receives the output from the upstream task, it keeps
%% track of the logical clock value associated with the output. The
%% logical clock value is used to identify the duplicate output. The
%% framework drops the output if there is an output with the same logical
%% clock value already pushed in the input queue of the downstream
%% task. To reduce the overhead of straggler mitigation, the framework
%% only maintains this additional per task record keeping in case when
%% straggler mitigation is happening for a task.

%% The traditional way of mitigating stragglers is by cloning the tasks~\cite{mantri}. However, cloning an NF task comes with two additional challenges. The first challenge is that a packet processing task may produce output on every packet, so simply mirroring the same input to the clone results in duplicate outputs - network traffic. Our framework as shown in \figref{fig-straggler}, overcomes this challenge by suppressing the duplicate output. When the downstream task receives the output from the upstream task, it keeps track of the logical clock value associated with the output. The logical clock value is used to identify the duplicate output. The framework drops the output if there is an output with the same logical clock value already pushed in the input queue of the downstream task. To reduce the overhead of straggler mitigation, the framework only maintains this additional per task record keeping in case when straggler mitigation is happening for a task.

%% \begin{figure}[h!]
%%     \begin{center}
%%     \includegraphics[width=0.45\textwidth]{figures/straggler.pdf}
%%     \caption{Duplication suppression}
%%     \label{fig-straggler}
%%     \end{center}        
%%\end{figure}

%% There are now two potential issues with duplicates. First,  Second, there can be duplicate updates to state by the
%% straggler and its clone. To address this, the datastore manager keeps
%% track of all the returned values of update operations associated with
%% the cloned input. When a second request (associated with the same
%% logical clock) is received for the update operation, we return the
%% value returned when the logical clock was last used in the
%% update.
%% Together these ideas help \name suppress various forms of
%% duplicates and support R5 without side-effects (i.e., impacting other
%% requirments).
%% Similar to fault tolerance, the datastore manager uses the
%% logical clock value to store and lookup the return value of the state
%% operation.

%% The framework monitors both the straggler and the clone, and
%% terminates the slowed one.


%% If the clone is faster and catches up with the straggler, the
%% framework kills the straggler. However, if it does not monitor any
%% improvement in the packet processing latency, it kills the clone.

%\subsection{Avoid packet re-parsing}
%\label{avoid-reparsing}
%Instead of re-parsing the packet at each worker, the worker registers for input types with the parser. The parser parses the packet headers to generate both low level and high level inputs (HTTP GET, TCP connection). If a worker registers for an event which one of the upstream workers; in the chain, has also registered for, then the downstream worker does not need to reparse the packet header to generate the same input. 

%For simple events like IP header or TCP connection hearder, the parser does not need to maintain any state. However, for more complex inputs, the parser needs to maintain state e.g. for HTTP segment, the parser has to parse and concatenate multiple TCP packets. In case of a failure of a parser this state needs to be regenerated. We leverage the fact that parser does not have any shared state and that we are already logging the input for fault tolerance purposes, so instead of storing the parser's state, we replay input packets to regenerate the state. 


==> paper - Copy/summary.tex <==
\section{Conclusion}

We presented a ground-up NFV framework called \name to support COE and
high performance for NFV chains. \name relies on managing state
external to NFs, but couples that with several caching and state
update algorithms to ensure low latency and high throughput. In
addition, it leverage simple metadata to ensure various correctness
properties are maintained even under traffic reallocation, NF
failures, as well as failures of key \name framework components.

%%    support is tedious, and is slowing down the wider adoption of
%%    NFV. Simplifying this process is key for wider proliferation of
%%    NFV. To this end, we design a generic, and network function
%%    independent framework that makes it easier for developers to build
%%    scalable and highly available NFs. We offload the complexity of
%%    providing these features to the framework at a minimal overhead,
%%    similar to frameworks for cloud computing applications.}
 
%\end{abstract}

%\phantomsection



==> paper - Copy/tables/duplicate_supression.tex <==
\begin{table}
\centering
\small
\setlength{\tabcolsep}{0.5em}
\begin{scriptsize}
\begin{tabular}{l||ccc}

&
25$\%$load&
50$\%$load&
75$\%$load\\

\hline
\hline
			
Duplicate packets & 9068 & 15346& 24051\\
Duplicate state updates & 187 & 429 & 661\\

\end{tabular}
\compactcaption{Duplicate packet and state update at the downstream port scan detector without duplicate suppression.}
\end{scriptsize}
\vspace{-1em}
\label{t:duplicate}
\end{table}


==> paper - Copy/tables/existing_frameworks.tex <==
\begin{table*}
	\centering
	\setlength{\tabcolsep}{0.85em}
	\begin{scriptsize}
		\begin{tabular}{lcccccccc}
			
			&
			({\em R1})&
			({\em R2})&
			({\em R3})&
			({\em R4})&
			({\em R5})&
			({\em R6})&
			& 
			\\
			
			
			&
			\bf State &
			\bf State &
			\bf State &
			\bf Chain wide &
			\bf Duplicate  &
			\bf Cross NF  & 
			\bf High &
			\bf Service \\
			%%
			\bf Framework &
			\bf availability &
			\bf transfer &
			\bf sharing &
			\bf ordering &
			\bf suppression &
			\bf analysis &
			\bf level APIs &
			\bf chaining\\
			
			\hline
			\hline
			
			E2~\cite{E2} & & & &  & & \cmark$^{1}$   &  \cmark & \cmark\\
			FlowTags~\cite{flowtags}  & & & & & & \cmark$^{1}$ &  & \cmark\\ 
			FTMB~\cite{ftmb} & \cmark & & & & & & & \\ 
			Pico~\cite{pico} & \cmark & & & & & & & \\ 
			OpenBox~\cite{OpenBox} & & & & & & \cmark$^{1}$  & & \cmark \\ 
			OpenNF~\cite{opennf} & \cmark$^{2}$ & \cmark &  \cmark$^{3}$ & & & & & \\
			SIMPLE~\cite{simple}  & & & & & & & & \cmark  \\
			Split/Merge~\cite{splitmerge}  & & \cmark &  \cmark$^{3}$ & & & & & \\
			Stateless NF~\cite{statelessnf}  & \cmark$^{4}$ & \cmark &  \cmark$^{3}$ & & & & &  \\
			PGA~\cite{PGA}  & & & & & & & \cmark & \cmark \\
			xOMB~\cite{xomb} & & & & &  & \cmark$^{1}$  &  & \cmark \\ 
			StreamNF & \cmark & \cmark & \cmark & \cmark & \cmark  & \cmark &\cmark & \cmark \\
			
		\end{tabular}
		
		
		%\end{scriptsize}
		%\begin{scriptsize}
		
		$^{1}$ Limited contextual information. $^{2}$Requires hot-standby. $^{3}$ High state sharing overhead.  $^{4}$Perform poorly for write-heavy state.
	\end{scriptsize}
	
	\caption{Existing NFV frameworks.\aditya{Table columns should be R1--R7 + ``Chaining'' + ``High-Level API''. Also list PGA}  \JK{updated the table} }
	\label{t:frameworks}
\end{table*}


==> paper - Copy/tables/multifailures.tex <==
\begin{table}
	\centering
	\setlength{\tabcolsep}{0.5em}
        \small
        	%\begin{scriptsize}
		\begin{tabular}{l||cc}
			&
			NF instance&
			Root\\
			
			\hline
			\hline
			
			Store instance & \cmark$^*$ & \cmark$^*$\\
			NF instance & \cmark &\cmark\\
			
		\end{tabular}
%		\vspace{-1em}
		\caption{Handling of correlated failures ($^*$Cannot recover if component and the store instance storing its state fail together).}
	%\end{scriptsize}
	\vspace{-1.2em}
\label{ts:mutliplefailures}	
\end{table}


==> paper - Copy/tables/operations.tex <==
\begin{table}
\centering
\footnotesize
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{p{2.4cm}|p{4.6cm}}

\textbf{Operation} & \textbf{Description} \\
\hline\hline
Increment/ decrement a value &  Increment or decrement the value stored at key by the given value.    \\ 
\hline
Push/pop a value to/from list & Push or pop the value in/from the list stored at the given key. \\% If the list does not exist, create a list.\\
\hline
Compare and update &  Update the value, if the condition is true.\\

\end{tabular}
\compactcaption{Basic operations offloaded to datastore manager}
\label{t:operations}
\vspace{-0.1in}
\end{table}


==> tables/duplicate_supression.tex <==
\begin{table}
\centering
\small
\setlength{\tabcolsep}{0.5em}
\begin{scriptsize}
\begin{tabular}{l||ccc}

&
25$\%$load&
50$\%$load&
75$\%$load\\

\hline
\hline
			
Duplicate packets & 9068 & 15346& 24051\\
Duplicate state updates & 187 & 429 & 661\\

\end{tabular}
\compactcaption{Duplicate packet and state update at the downstream port scan detector without duplicate suppression.}
\end{scriptsize}
\vspace{-1em}
\label{t:duplicate}
\end{table}


==> tables/existing_frameworks.tex <==
\begin{table*}
	\centering
	\setlength{\tabcolsep}{0.85em}
	\begin{scriptsize}
		\begin{tabular}{lcccccccc}
			
			&
			({\em R1})&
			({\em R2})&
			({\em R3})&
			({\em R4})&
			({\em R5})&
			({\em R6})&
			& 
			\\
			
			
			&
			\bf State &
			\bf State &
			\bf State &
			\bf Chain wide &
			\bf Duplicate  &
			\bf Cross NF  & 
			\bf High &
			\bf Service \\
			%%
			\bf Framework &
			\bf availability &
			\bf transfer &
			\bf sharing &
			\bf ordering &
			\bf suppression &
			\bf analysis &
			\bf level APIs &
			\bf chaining\\
			
			\hline
			\hline
			
			E2~\cite{E2} & & & &  & & \cmark$^{1}$   &  \cmark & \cmark\\
			FlowTags~\cite{flowtags}  & & & & & & \cmark$^{1}$ &  & \cmark\\ 
			FTMB~\cite{ftmb} & \cmark & & & & & & & \\ 
			Pico~\cite{pico} & \cmark & & & & & & & \\ 
			OpenBox~\cite{OpenBox} & & & & & & \cmark$^{1}$  & & \cmark \\ 
			OpenNF~\cite{opennf} & \cmark$^{2}$ & \cmark &  \cmark$^{3}$ & & & & & \\
			SIMPLE~\cite{simple}  & & & & & & & & \cmark  \\
			Split/Merge~\cite{splitmerge}  & & \cmark &  \cmark$^{3}$ & & & & & \\
			Stateless NF~\cite{statelessnf}  & \cmark$^{4}$ & \cmark &  \cmark$^{3}$ & & & & &  \\
			PGA~\cite{PGA}  & & & & & & & \cmark & \cmark \\
			xOMB~\cite{xomb} & & & & &  & \cmark$^{1}$  &  & \cmark \\ 
			StreamNF & \cmark & \cmark & \cmark & \cmark & \cmark  & \cmark &\cmark & \cmark \\
			
		\end{tabular}
		
		
		%\end{scriptsize}
		%\begin{scriptsize}
		
		$^{1}$ Limited contextual information. $^{2}$Requires hot-standby. $^{3}$ High state sharing overhead.  $^{4}$Perform poorly for write-heavy state.
	\end{scriptsize}
	
	\caption{Existing NFV frameworks.\aditya{Table columns should be R1--R7 + ``Chaining'' + ``High-Level API''. Also list PGA}  \JK{updated the table} }
	\label{t:frameworks}
\end{table*}

